Geometry-Based Channel Estimation, Prediction, and Fusion

Reciprocity-based beamforming-most commonly employed in time-division duplexing-uses noisy, estimated (i.e., measured) channel state information (CSI) acquired on the uplink. While computationally efficient, reciprocity-based beamforming suffers severe losses under (i) low signal-to-noise ratio (SNR) and (ii) user mobility because it ignores the underlying physics of the radio channel beyond its reciprocity. Based on a physics-driven geometry-based channel model, we propose a method that jointly infers the mobile user's position and environment map on the uplink. It then leverages the estimated user position and environment map to predict CSI on the downlink. We demonstrate significant efficiency gains under both (i) low SNR and (ii) user mobility on measured data. While the user position may allow efficient beamforming in strong line-of-sight (LoS) channels, inferring an environment map allows bypassing obstructed LoS conditions using non-LoS beamforming via multipath components. We further propose "channel fusion," a probabilistic (Bayesian) combination of estimated and predicted CSI, which increases the beamforming robustness, particularly when either source of CSI is unreliable. Notably, this approach shares similarities with the minimum mean square error (MMSE) channel estimator, with geometry-based prior parameters inferred from the data.

==> IEEEabrv.tex <==
journal = IEEE_J_AC,
@STRING{IEEE_J_ANNE = "{IEEE} Trans. Aeronaut. Navig. Electron."}
@STRING{IEEE_J_AES = "{IEEE} Trans. Aerosp. Electron. Syst."}
@STRING{IEEE_J_ANE = "{IEEE} Trans. Aerosp. Navig. Electron."}
@STRING{IEEE_J_AS = "{IEEE} Trans. Aerosp."}
@STRING{IEEE_J_AIRE = "{IEEE} Trans. Airborne Electron."}
@STRING{IEEE_J_MIL = "{IEEE} Trans. Mil. Electron."}
@STRING{IEEE_J_ITS = "{IEEE} Trans. Intell. Transp. Syst."}
@STRING{IEEE_J_IV = "{IEEE} Trans. Intell. Veh."}
@STRING{IEEE_J_TTE = "{IEEE} Trans. Transport. Electrific."}
@STRING{IEEE_J_VC = "{IEEE} Trans. Veh. Commun."}
@STRING{IEEE_J_VT = "{IEEE} Trans. Veh. Technol."}
@STRING{IEEE_J_STSP = "{IEEE} J. Sel. Topics Signal Process."}
@STRING{IEEE_J_SPL = "{IEEE} Signal Process. Lett."}
@STRING{IEEE_J_SYST = "{IEEE} Syst. J."}
@STRING{IEEE_J_ASSP = "{IEEE} Trans. Acoust., Speech, Signal Process."}
@STRING{IEEE_J_AU = "{IEEE} Trans. Audio"}
@STRING{IEEE_J_AUEA = "{IEEE} Trans. Audio Electroacoust."}
@STRING{IEEE_J_ASLP = "{IEEE/ACM} Trans. Audio, Speech, Language Process."}
@STRING{IEEE_J_ASL = "{IEEE} Audio, Speech, Language Process."}
@STRING{IEEE_J_AC = "{IEEE} Trans. Autom. Control"}
@STRING{IEEE_J_CAS = "{IEEE} Trans. Circuits Syst."}
@STRING{IEEE_J_CASVT = "{IEEE} Trans. Circuits Syst. Video Technol."}
@STRING{IEEE_J_CASI = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CASI_RP = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII_EB = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CT = "{IEEE} Trans. Circuit Theory"}
@STRING{IEEE_J_CST = "{IEEE} Trans. Control Syst. Technol."}
@STRING{IEEE_J_ETCAS = "{IEEE} Trans. Emerg. Sel. Topics Circuits Syst."}
@STRING{IEEE_J_SP = "{IEEE} Trans. Signal Process."}
@STRING{IEEE_J_SU = "{IEEE} Trans. Sonics Ultrason."}
@STRING{IEEE_J_SAP = "{IEEE} Trans. Speech Audio Process."}
@STRING{IEEE_J_UE = "{IEEE} Trans. Ultrason. Eng."}
@STRING{IEEE_J_UFFC = "{IEEE} Trans. Ultrason., Ferroelectr., Freq. Control"}
@STRING{IEEE_J_COML = "{IEEE} Commun. Lett."}
@STRING{IEEE_J_JSAC = "{IEEE} J. Sel. Areas Commun."}
@STRING{IEEE_J_COM = "{IEEE} Trans. Commun."}
@STRING{IEEE_J_COMT = "{IEEE} Trans. Commun. Technol."}
@STRING{IEEE_J_WCOM = "{IEEE} Trans. Wireless Commun."}
@STRING{IEEE_J_WCOML = "{IEEE} Wireless Commun. Lett."}
@STRING{IEEE_J_ADVP = "{IEEE} Trans. Adv. Packag."}
@STRING{IEEE_J_CHMT = "{IEEE} Trans. Compon., Hybrids, Manuf. Technol."}
@STRING{IEEE_J_CPMT = "{IEEE} Trans. Compon. Packag. Manuf. Technol."}
@STRING{IEEE_J_CPMTA = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {A}"}
@STRING{IEEE_J_CPMTB = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {B}"}
@STRING{IEEE_J_CPMTC = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {C}"}
@STRING{IEEE_J_CAPTS = "{IEEE} Trans. Compon. Packag. Technol."}
@STRING{IEEE_J_CAPT = "{IEEE} Trans. Compon. Packag. Technol."}
@STRING{IEEE_J_CPART = "{IEEE} Trans. Compon. Parts"}
@STRING{IEEE_J_EPM = "{IEEE} Trans. Electron. Packag. Manuf."}
@STRING{IEEE_J_MFT = "{IEEE} Trans. Manuf. Technol."}
@STRING{IEEE_J_PHP = "{IEEE} Trans. Parts, Hybrids, Packag."}
@STRING{IEEE_J_PMP = "{IEEE} Trans. Parts, Mater., Packag."}
@STRING{IEEE_J_TCAD = "{IEEE} J. Technol. Comput. Aided Design"}
@STRING{IEEE_J_CAD = "{IEEE} Trans. Comput.-Aided Design Integr. Circuits Syst."}
@STRING{IEEE_J_BD = "{IEEE} Trans. Big Data"}
@STRING{IEEE_J_IFS = "{IEEE} Trans. Inf. Forensics Security"}
@STRING{IEEE_J_IT = "{IEEE} Trans. Inf. Theory"}
@STRING{IEEE_J_KDE = "{IEEE} Trans. Knowl. Data Eng."}
@STRING{IEEE_J_CAL = "{IEEE} Comput. Archit. Lett."}
@STRING{IEEE_J_ES = "{IEEE} Embedded Syst. Lett."}
@STRING{IEEE_J_IOT = "{IEEE} Internet Things J."}
@STRING{IEEE_J_XCDC = "{IEEE} J. Explor. Solid-State Computat. Devices Circuits"}
@STRING{IEEE_J_MMCT = "{IEEE} J. Multiscale and Multiphys. Comput. Techn."}
@STRING{IEEE_J_SUSC = "{IEEE} Sustain. Comput."}
@STRING{IEEE_J_CC = "{IEEE} Trans. on Cloud Comput."}
@STRING{IEEE_J_CSS = "{IEEE} Trans. Comput. Social Syst."}
@STRING{IEEE_J_C = "{IEEE} Trans. Comput."}
@STRING{IEEE_J_CNS = "{IEEE} Trans. Control Netw. Syst."}
@STRING{IEEE_J_DSC = "{IEEE} Trans. Depend. Sec. Comput."}
@STRING{IEEE_J_ECOMP = "{IEEE} Trans. Electron. Comput."}
@STRING{IEEE_J_ETC = "{IEEE} Trans. Emerg. Topics Comput."}
@STRING{IEEE_J_EVC = "{IEEE} Trans. Evol. Comput."}
@STRING{IEEE_J_FUZZ = "{IEEE} Trans. Fuzzy Syst."}
@STRING{IEEE_J_MC = "{IEEE} Trans. Mobile Comput."}
@STRING{IEEE_J_MSCS = "{IEEE} Trans. Multi-Scale Comput. Syst."}
@STRING{IEEE_J_NET = "{IEEE/ACM} Trans. Netw."}
@STRING{IEEE_J_NSE = "{IEEE} Trans. Netw. Sci. Eng."}
@STRING{IEEE_J_NSM = "{IEEE} Trans. Netw. Service Manag."}
@STRING{IEEE_J_NN = "{IEEE} Trans. Neural Netw."}
@STRING{IEEE_J_NNLS = "{IEEE} Trans. Neural Netw. Learn. Syst."}
@STRING{IEEE_J_PDS = "{IEEE} Trans. Parallel Distrib. Syst."}
@STRING{IEEE_J_SC = "{IEEE} Trans. Serv. Comput."}
@STRING{IEEE_J_SIPN = "{IEEE} Trans. Signal Inf. Process. Netw."}
@STRING{IEEE_J_SE = "{IEEE} Trans. Softw. Eng."}
@STRING{IEEE_J_JDT = "{IEEE/OSA} J. Display Technol."}
@STRING{IEEE_J_IP = "{IEEE} Trans. Image Process."}
@STRING{IEEE_J_MM = "{IEEE} Trans. Multimedia"}
@STRING{IEEE_J_VCG = "{IEEE} Trans. Vis. Comput. Graphics"}
@STRING{IEEE_J_JAS = "{IEEE/CAA} J. Autom. Sinica"}
@STRING{IEEE_J_JRA = "{IEEE} J. Robot. Autom."}
@STRING{IEEE_J_AFFC = "{IEEE} Trans. Affect. Comput."}
@STRING{IEEE_J_ASE = "{IEEE} Trans. Autom. Sci. Eng."}
@STRING{IEEE_J_AMD = "{IEEE} Trans. Auton. Mental Develop."}
@STRING{IEEE_J_CCN = "{IEEE} Trans. on Cogn. Commun. Netw."}
@STRING{IEEE_J_CDS = "{IEEE} Trans. Cogn. Develop. Syst."}
@STRING{IEEE_J_CIAIG = "{IEEE} Trans. Comput. Intell. {AI} in Games"}
@STRING{IEEE_J_CYB = "{IEEE} Trans. Cybern."}
@STRING{IEEE_J_H = "{IEEE} Trans. Haptics"}
@STRING{IEEE_J_HFE = "{IEEE} Trans. Hum. Factors Electron."}
@STRING{IEEE_J_HMS = "{IEEE} Trans. Human-Mach. Syst."}
@STRING{IEEE_J_MMS = "{IEEE} Trans. Man-Mach. Syst."}
@STRING{IEEE_J_PAMI = "{IEEE} Trans. Pattern Anal. Mach. Intell."}
@STRING{IEEE_J_RA = "{IEEE} Trans. Robot. Autom."}
@STRING{IEEE_J_RAL = "{IEEE} Robot. Autom. Lett."}
@STRING{IEEE_J_RO = "{IEEE} Trans. Robot."}
@STRING{IEEE_J_SMC = "{IEEE} Trans. Syst., Man, Cybern."}
@STRING{IEEE_J_SMCA = "{IEEE} Trans. Syst., Man, Cybern. {A}"}
@STRING{IEEE_J_SMCB = "{IEEE} Trans. Syst., Man, Cybern. {B}"}
@STRING{IEEE_J_SMCC = "{IEEE} Trans. Syst., Man, Cybern. {C}"}
@STRING{IEEE_J_SMCS = "{IEEE} Trans. Syst., Man, Cybern., Syst."}
@STRING{IEEE_J_SSC = "{IEEE} Trans. Syst. Sci. Cybern."}
@STRING{IEEE_J_GRSL = "{IEEE} Geosci. Remote Sens. Lett."}
@STRING{IEEE_J_GE = "{IEEE} Trans. Geosci. Electron."}
@STRING{IEEE_J_GRS = "{IEEE} Trans. Geosci. Remote Sens."}
@STRING{IEEE_J_OE = "{IEEE} J. Ocean. Eng."}
@STRING{IEEE_J_STARS = "{IEEE} J. Sel. Topics Appl. Earth Observ. Remote Sens."}
@STRING{IEEE_J_CJECE = "Canadian J. Elect. Comput. Eng."}
@STRING{IEEE_J_PROC = "Proc. {IEEE}"}
@STRING{IEEE_J_RITA = "{IEEE} Revista Iberoamericana de Technolog{\'{i}}as del Aprendizaje"}
@STRING{IEEE_J_EDU = "{IEEE} Trans. Educ."}
@STRING{IEEE_J_EM = "{IEEE} Trans. Eng. Manag."}
@STRING{IEEE_J_EWS = "{IEEE} Trans. Eng. Writing Speech"}
@STRING{IEEE_J_LT = "{IEEE} Trans. Learn. Technol."}
@STRING{IEEE_J_PC = "{IEEE} Trans. Prof. Commun."}
@STRING{IEEE_J_AWPL = "{IEEE} Antennas Wireless Propag. Lett."}
@STRING{IEEE_J_MAGL = "{IEEE} Magn. Lett."}
@STRING{IEEE_J_MGWL = "{IEEE} Microw. Guided Wave Lett."}
@STRING{IEEE_J_MWCL = "{IEEE} Microw. Wireless Compon. Lett."}
@STRING{IEEE_J_RFIC = "{IEEE} {RFIC} J."}
@STRING{IEEE_J_RFID = "{IEEE} {RFID} J."}
@STRING{IEEE_J_AP = "{IEEE} Trans. Antennas Propag."}
@STRING{IEEE_J_EMC = "{IEEE} Trans. Electromagn. Compat."}
@STRING{IEEE_J_MAG = "{IEEE} Trans. Magn."}
@STRING{IEEE_J_MTT = "{IEEE} Trans. Microw. Theory Techn."}
@STRING{IEEE_J_RFI = "{IEEE} Trans. Radio Freq. Interference"}
@STRING{IEEE_J_TTHZ = "{IEEE} Trans. {THz} Sci. Technol."}
@STRING{IEEE_J_TJMJ = "{IEEE} Transl. J. Magn. Jpn."}
@STRING{IEEE_J_PHOT = "{IEEE} J. Photovolt."}
@STRING{IEEE_J_PEL = "{IEEE} Power Electron. Lett."}
@STRING{IEEE_J_PETS = "{IEEE} Power Energy Technol. Syst. J."}
@STRING{IEEE_J_ESTPE = "{IEEE} Trans. Emerg. Sel. Topics Power Electron."}
@STRING{IEEE_J_EC = "{IEEE} Trans. Energy Convers."}
@STRING{IEEE_J_PWRAS = "{IEEE} Trans. Power App. Syst."}
@STRING{IEEE_J_PWRD = "{IEEE} Trans. Power Del."}
@STRING{IEEE_J_PWRE = "{IEEE} Trans. Power Electron."}
@STRING{IEEE_J_PWRS = "{IEEE} Trans. Power Syst."}
@STRING{IEEE_J_SG = "{IEEE} Trans. Smart Grid"}
@STRING{IEEE_J_STE = "{IEEE} Trans. Sustain. Energy"}
@STRING{IEEE_J_PSE = "{IEEE} J. Product Safety Eng."}
@STRING{IEEE_J_APPIND = "{IEEE} Trans. Appl. Ind."}
@STRING{IEEE_J_BC = "{IEEE} Trans. Broadcast."}
@STRING{IEEE_J_BCTV = "{IEEE} Trans. Broadcast Television Receivers"}
@STRING{IEEE_J_CE = "{IEEE} Trans. Consum. Electron."}
@STRING{IEEE_J_IE = "{IEEE} Trans. Ind. Electron."}
@STRING{IEEE_J_IECI = "{IEEE} Trans. Ind. Electron. Contr. Instrum."}
@STRING{IEEE_J_IA = "{IEEE} Trans. Ind. Appl."}
@STRING{IEEE_J_IGA = "{IEEE} Trans. Ind. Gen. Appl."}
@STRING{IEEE_J_IINF = "{IEEE} Trans. Ind. Informat."}
@STRING{IEEE_J_IM = "{IEEE} Trans. Instrum. Meas."}
@STRING{IEEE_J_JEM = "{IEEE/TMS} J. Electron. Mater."}
@STRING{IEEE_J_DEI = "{IEEE} Trans. Dielectr. Electr. Insul."}
@STRING{IEEE_J_EI = "{IEEE} Trans. Electr. Insul."}
@STRING{IEEE_J_MEMS = "J. Microelectromech. Syst."}
@STRING{IEEE_J_MEMSI = "J. Microelectromech. Syst."}
@STRING{IEEE_J_MECH = "{IEEE/ASME} Trans. Mechatronics"}
@STRING{IEEE_J_BHI = "{IEEE} J. Biomed. Health Inform."}
@STRING{IEEE_J_TEHM = "{IEEE} J. Transl. Eng. Health Med."}
@STRING{IEEE_J_LS = "{IEEE} Life Sci. Lett."}
@STRING{IEEE_J_RBME = "{IEEE} Rev. Biomed. Eng."}
@STRING{IEEE_J_BCAS = "{IEEE} Trans. Biomed. Circuits Syst."}
@STRING{IEEE_J_BMELC = "{IEEE} Trans. Bio-Med. Electron."}
@STRING{IEEE_J_BME = "{IEEE} Trans. Biomed. Eng."}
@STRING{IEEE_J_B-ME = "{IEEE} Trans. Bio-Med. Eng."}
@STRING{IEEE_J_CBB = "{IEEE/ACM} Trans. Comput. Biol. Bioinformatics"}
@STRING{IEEE_J_ITBM = "{IEEE} Trans. Inf. Technol. Biomed."}
@STRING{IEEE_J_ME = "{IEEE} Trans. Med. Electron."}
@STRING{IEEE_J_MI = "{IEEE} Trans. Med. Imag."}
@STRING{IEEE_J_MBSC = "{IEEE} Trans. Mol. Biol. Multi-Scale Commun."}
@STRING{IEEE_J_NB = "{IEEE} Trans. Nanobiosci."}
@STRING{IEEE_J_NSRE = "{IEEE} Trans. Neural Syst. Rehabil. Eng."}
@STRING{IEEE_J_RE = "{IEEE} Trans. Rehabil. Eng."}
@STRING{IEEE_J_JLT = "J. Lightw. Technol."}
@STRING{IEEE_J_OCN = "{IEEE} J. Opt. Commun. Netw."}
@STRING{IEEE_J_PJ = "{IEEE} Photon. J."}
@STRING{IEEE_J_PTL = "{IEEE} Photon. Technol. Lett."}
@STRING{IEEE_J_EDL = "{IEEE} Electron Device Lett."}
@STRING{IEEE_J_EDS = "{IEEE} J. Electron Devices Soc."}
@STRING{IEEE_J_JQE = "{IEEE} J. Quantum Electron."}
@STRING{IEEE_J_JSTQE = "{IEEE} J. Sel. Topics Quantum Electron."}
@STRING{IEEE_J_ENANO = "{IEEE} Nanotechnol. Express"}
@STRING{IEEE_J_ED = "{IEEE} Trans. Electron Devices"}
@STRING{IEEE_J_NANO = "{IEEE} Trans. Nanotechnol."}
@STRING{IEEE_J_NS = "{IEEE} Trans. Nucl. Sci."}
@STRING{IEEE_J_PS = "{IEEE} Trans. Plasma Sci."}
@STRING{IEEE_J_DMR = "{IEEE} Trans. Device Mater. Rel."}
@STRING{IEEE_J_R = "{IEEE} Trans. Rel."}
@STRING{IEEE_J_ESSL = "{IEEE/ECS} Electrochem. Solid-State Lett."}
@STRING{IEEE_J_JSSC = "{IEEE} J. Solid-State Circuits"}
@STRING{IEEE_J_ASC = "{IEEE} Trans. Appl. Supercond."}
@STRING{IEEE_J_SM = "{IEEE} Trans. Semicond. Manuf."}
@STRING{IEEE_J_SENSOR = "{IEEE} Sensors J."}
@STRING{IEEE_J_VLSI = "{IEEE} Trans. {VLSI} Syst."}
@STRING{IEEE_O_ACC = "{IEEE} Access"}
@STRING{IEEE_M_AES = "{IEEE} Aerosp. Electron. Syst. Mag."}
@STRING{IEEE_M_HIST = "{IEEE} Ann. Hist. Comput."}
@STRING{IEEE_M_AP = "{IEEE} Antennas Propag. Mag."}
@STRING{IEEE_M_ASSP = "{IEEE} {ASSP} Mag."}
@STRING{IEEE_M_CHINAC = "China Commun."}
@STRING{IEEE_M_CD = "{IEEE} Circuits Devices Mag."}
@STRING{IEEE_M_CAS = "{IEEE} Circuits Syst. Mag."}
@STRING{IEEE_M_COM = "{IEEE} Commun. Mag."}
@STRING{IEEE_M_COMSOC = "{IEEE} Commun. Soc. Mag."}
@STRING{IEEE_O_CSTO = "{IEEE} Commun. Surveys Tuts."}
@STRING{IEEE_M_CIM = "{IEEE} Comput. Intell. Mag."}
@STRING{IEEE_M_CSE = "{IEEE} Comput. Sci. Eng."}
@STRING{IEEE_M_CSEM = "{IEEE} Comput. Sci. Eng. Mag."}
@STRING{IEEE_M_C = "Computer"}
@STRING{IEEE_M_CAP = "{IEEE} Comput. Appl. Power"}
@STRING{IEEE_M_CGA = "{IEEE} Comput. Graph. Appl."}
@STRING{IEEE_M_CONC = "{IEEE} Concurrency"}
@STRING{IEEE_M_CS = "{IEEE} Control Syst. Mag."}
@STRING{IEEE_M_DT = "{IEEE} Des. Test"}
@STRING{IEEE_M_DTC = "{IEEE} Des. Test. Comput."}
@STRING{IEEE_O_DSO = "{IEEE} Distrib. Syst. Online"}
@STRING{IEEE_M_EI = "{IEEE} Electr. Insul. Mag."}
@STRING{IEEE_M_ETF = "{IEEE} Electrific. Mag."}
@STRING{IEEE_M_EMC = "{IEEE} Electromagn. Compat."}
@STRING{IEEE_M_ETR = "{IEEE} ElectroTechnol. Rev."}
@STRING{IEEE_M_EMR = "{IEEE} Eng. Manag. Rev."}
@STRING{IEEE_M_EMB = "{IEEE} Eng. Med. Biol. Mag."}
@STRING{IEEE_M_EXP = "{IEEE} Expert"}
@STRING{IEEE_M_GRS = "{IEEE} Geosci. Remote Sens. Mag."}
@STRING{IEEE_M_IA = "{IEEE} Ind. Appl. Mag."}
@STRING{IEEE_M_IE = "{IEEE} Ind. Electron. Mag."}
@STRING{IEEE_M_IM = "{IEEE} Instrum. Meas. Mag."}
@STRING{IEEE_M_IS = "{IEEE} Intell. Syst."}
@STRING{IEEE_M_ITS = "{IEEE} Intell. Transp. Syst. Mag."}
@STRING{IEEE_M_IC = "{IEEE} Internet Comput."}
@STRING{IEEE_M_ITP = "{IEEE} {IT} Prof."}
@STRING{IEEE_M_MICRO = "{IEEE} Micro"}
@STRING{IEEE_M_MW = "{IEEE} Microw. Mag."}
@STRING{IEEE_M_MM = "{IEEE} Multimedia"}
@STRING{IEEE_M_NANO = "{IEEE} Nanotechnol. Mag."}
@STRING{IEEE_M_NET = "{IEEE} Netw."}
@STRING{IEEE_M_PCOM = "{IEEE} Personal Commun. Mag."}
@STRING{IEEE_M_PVC = "{IEEE} Pervasive Comput."}
@STRING{IEEE_M_POT = "{IEEE} Potentials"}
@STRING{IEEE_M_PEL = "{IEEE} Power Electron. Mag."}
@STRING{IEEE_M_PE = "{IEEE} Power Energy Mag."}
@STRING{IEEE_M_PER = "{IEEE} Power Eng. Rev."}
@STRING{IEEE_M_PULSE = "{IEEE} Pulse"}
@STRING{IEEE_M_RA = "{IEEE} Robot. Autom. Mag."}
@STRING{IEEE_M_SAP = "{IEEE} Security Privacy"}
@STRING{IEEE_M_SP = "{IEEE} Signal Process. Mag."}
@STRING{IEEE_M_S = "{IEEE} Softw."}
@STRING{IEEE_M_SSC = "{IEEE} Solid-State Circuits Mag."}
@STRING{IEEE_M_SPECT = "{IEEE} Spectr."}
@STRING{IEEE_M_SMC = "{IEEE} Syst., Man, Cybern. Mag."}
@STRING{IEEE_M_TS = "{IEEE} Technol. Soc. Mag."}
@STRING{IEEE_M_VT = "{IEEE} Veh. Technol. Mag."}
@STRING{IEEE_M_WC = "{IEEE} Wireless Commun."}
@STRING{IEEE_M_TODAY = "Today's Engineer"}


==> figures/channel-fusion-shadows.tex <==
\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
111	-35.5669502794439\\
112	-36.0924320435732\\
113	-36.351475336133\\
114	-36.8479511671828\\
115	-37.0632116240475\\
116	-37.0661319571525\\
117	-37.2588816303491\\
118	-37.3990845639327\\
119	-37.5570851885126\\
120	-37.7057218158072\\
121	-37.5588812762327\\
122	-38.2536505185237\\
123	-38.5534615708318\\
124	-39.1976275498693\\
125	-39.4582077510982\\
126	-39.3643484163815\\
127	-39.9526374505114\\
128	-40.3569876273323\\
129	-39.4236330039063\\
130	-40.1975152983885\\
131	-40.1591960960801\\
132	-39.2141563845845\\
133	-39.6009047321718\\
134	-39.9876530797592\\
135	-40.5695678694775\\
136	-41.2810930139678\\
137	-40.7254448885807\\
138	-40.8653355994745\\
139	-40.517168397127\\
140	-41.1436300938016\\
141	-41.2916902925916\\
142	-41.100108632918\\
143	-41.0791236015771\\
144	-40.6120066609437\\
145	-39.7632521134971\\
146	-39.8505505835477\\
147	-40.1249030448183\\
148	-39.9158992879064\\
149	-39.5932387658054\\
150	-40.4875413625722\\
151	-40.3172237143515\\
152	-40.7079864610304\\
153	-40.7350492396635\\
154	-40.6405032241364\\
155	-40.3651494224422\\
156	-40.1504630705807\\
157	-39.5272836073848\\
158	-38.792267653329\\
159	-38.4272287460992\\
160	-38.9561853424272\\
161	-40.0974078951085\\
162	-40.1266722263973\\
163	-39.785689070857\\
164	-39.3904635518935\\
165	-39.4364553823933\\
166	-38.7675161819392\\
167	-38.9392219463423\\
168	-38.4464370548603\\
169	-37.4414093010701\\
170	-36.8384211722961\\
171	-37.763299139291\\
172	-37.9953742137359\\
173	-37.2637013325052\\
174	-37.2413400328124\\
175	-36.9997889800459\\
176	-37.0045095268116\\
177	-36.7014700875858\\
178	-36.4261339843527\\
179	-36.6205927259132\\
180	-37.6861166571578\\
181	-37.6211364131236\\
182	-37.9234369673119\\
183	-37.5037586079944\\
184	-37.582782578722\\
185	-37.1524975796374\\
186	-36.5394020603518\\
187	-36.4335351305984\\
188	-37.3211832814352\\
189	-37.2695783357305\\
190	-36.5987594916508\\
191	-36.9452518608838\\
192	-37.0575693476256\\
193	-37.0447842238401\\
194	-35.9571248887183\\
195	-35.7643377897755\\
196	-36.7204901514943\\
197	-36.4383174146219\\
198	-36.505762030719\\
199	-35.9666430800494\\
199	-35.9666430800494\\
199	-25\\
111	-25\\
111	-35.5669502794439\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
111	-35.5669502794439\\
112	-36.0924320435732\\
113	-36.351475336133\\
114	-36.8479511671828\\
115	-37.0632116240475\\
116	-37.0661319571525\\
117	-37.2588816303491\\
118	-37.3990845639327\\
119	-37.5570851885126\\
120	-37.7057218158072\\
121	-37.5588812762327\\
122	-38.2536505185237\\
123	-38.5534615708318\\
124	-39.1976275498693\\
125	-39.4582077510982\\
126	-39.3643484163815\\
127	-39.9526374505114\\
128	-40.3569876273323\\
129	-39.4236330039063\\
130	-40.1975152983885\\
131	-40.1591960960801\\
132	-39.2141563845845\\
133	-39.6009047321718\\
134	-39.9876530797592\\
135	-40.5695678694775\\
136	-41.2810930139678\\
137	-40.7254448885807\\
138	-40.8653355994745\\
139	-40.517168397127\\
140	-41.1436300938016\\
141	-41.2916902925916\\
142	-41.100108632918\\
143	-41.0791236015771\\
144	-40.6120066609437\\
145	-39.7632521134971\\
146	-39.8505505835477\\
147	-40.1249030448183\\
148	-39.9158992879064\\
149	-39.5932387658054\\
150	-40.4875413625722\\
151	-40.3172237143515\\
152	-40.7079864610304\\
153	-40.7350492396635\\
154	-40.6405032241364\\
155	-40.3651494224422\\
156	-40.1504630705807\\
157	-39.5272836073848\\
158	-38.792267653329\\
159	-38.4272287460992\\
160	-38.9561853424272\\
161	-40.0974078951085\\
162	-40.1266722263973\\
163	-39.785689070857\\
164	-39.3904635518935\\
165	-39.4364553823933\\
166	-38.7675161819392\\
167	-38.9392219463423\\
168	-38.4464370548603\\
169	-37.4414093010701\\
170	-36.8384211722961\\
171	-37.763299139291\\
172	-37.9953742137359\\
173	-37.2637013325052\\
174	-37.2413400328124\\
175	-36.9997889800459\\
176	-37.0045095268116\\
177	-36.7014700875858\\
178	-36.4261339843527\\
179	-36.6205927259132\\
180	-37.6861166571578\\
181	-37.6211364131236\\
182	-37.9234369673119\\
183	-37.5037586079944\\
184	-37.582782578722\\
185	-37.1524975796374\\
186	-36.5394020603518\\
187	-36.4335351305984\\
188	-37.3211832814352\\
189	-37.2695783357305\\
190	-36.5987594916508\\
191	-36.9452518608838\\
192	-37.0575693476256\\
193	-37.0447842238401\\
194	-35.9571248887183\\
195	-35.7643377897755\\
196	-36.7204901514943\\
197	-36.4383174146219\\
198	-36.505762030719\\
199	-35.9666430800494\\
199	-35.9666430800494\\
199	-25\\
111	-25\\
111	-35.5669502794439\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
111	-35.5669502794439\\
112	-36.0924320435732\\
113	-36.351475336133\\
114	-36.8479511671828\\
115	-37.0632116240475\\
116	-37.0661319571525\\
117	-37.2588816303491\\
118	-37.3990845639327\\
119	-37.5570851885126\\
120	-37.7057218158072\\
121	-37.5588812762327\\
122	-38.2536505185237\\
123	-38.5534615708318\\
124	-39.1976275498693\\
125	-39.4582077510982\\
126	-39.3643484163815\\
127	-39.9526374505114\\
128	-40.3569876273323\\
129	-39.4236330039063\\
130	-40.1975152983885\\
131	-40.1591960960801\\
132	-39.2141563845845\\
133	-39.6009047321718\\
134	-39.9876530797592\\
135	-40.5695678694775\\
136	-41.2810930139678\\
137	-40.7254448885807\\
138	-40.8653355994745\\
139	-40.517168397127\\
140	-41.1436300938016\\
141	-41.2916902925916\\
142	-41.100108632918\\
143	-41.0791236015771\\
144	-40.6120066609437\\
145	-39.7632521134971\\
146	-39.8505505835477\\
147	-40.1249030448183\\
148	-39.9158992879064\\
149	-39.5932387658054\\
150	-40.4875413625722\\
151	-40.3172237143515\\
152	-40.7079864610304\\
153	-40.7350492396635\\
154	-40.6405032241364\\
155	-40.3651494224422\\
156	-40.1504630705807\\
157	-39.5272836073848\\
158	-38.792267653329\\
159	-38.4272287460992\\
160	-38.9561853424272\\
161	-40.0974078951085\\
162	-40.1266722263973\\
163	-39.785689070857\\
164	-39.3904635518935\\
165	-39.4364553823933\\
166	-38.7675161819392\\
167	-38.9392219463423\\
168	-38.4464370548603\\
169	-37.4414093010701\\
170	-36.8384211722961\\
171	-37.763299139291\\
172	-37.9953742137359\\
173	-37.2637013325052\\
174	-37.2413400328124\\
175	-36.9997889800459\\
176	-37.0045095268116\\
177	-36.7014700875858\\
178	-36.4261339843527\\
179	-36.6205927259132\\
180	-37.6861166571578\\
181	-37.6211364131236\\
182	-37.9234369673119\\
183	-37.5037586079944\\
184	-37.582782578722\\
185	-37.1524975796374\\
186	-36.5394020603518\\
187	-36.4335351305984\\
188	-37.3211832814352\\
189	-37.2695783357305\\
190	-36.5987594916508\\
191	-36.9452518608838\\
192	-37.0575693476256\\
193	-37.0447842238401\\
194	-35.9571248887183\\
195	-35.7643377897755\\
196	-36.7204901514943\\
197	-36.4383174146219\\
198	-36.505762030719\\
199	-35.9666430800494\\
199	-35.9666430800494\\
199	-25\\
111	-25\\
111	-35.5669502794439\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
113	-36.351475336133\\
114	-36.8479511671828\\
115	-37.0632116240475\\
116	-37.0661319571525\\
117	-37.2588816303491\\
118	-37.3990845639327\\
119	-37.5570851885126\\
120	-37.7057218158072\\
121	-37.5588812762327\\
122	-38.2536505185237\\
123	-38.5534615708318\\
124	-39.1976275498693\\
125	-39.4582077510982\\
126	-39.3643484163815\\
127	-39.9526374505114\\
128	-40.3569876273323\\
129	-39.4236330039063\\
130	-40.1975152983885\\
131	-40.1591960960801\\
132	-39.2141563845845\\
133	-39.6009047321718\\
134	-39.9876530797592\\
135	-40.5695678694775\\
136	-41.2810930139678\\
137	-40.7254448885807\\
138	-40.8653355994745\\
139	-40.517168397127\\
140	-41.1436300938016\\
141	-41.2916902925916\\
142	-41.100108632918\\
143	-41.0791236015771\\
144	-40.6120066609437\\
145	-39.7632521134971\\
146	-39.8505505835477\\
147	-40.1249030448183\\
148	-39.9158992879064\\
149	-39.5932387658054\\
150	-40.4875413625722\\
151	-40.3172237143515\\
152	-40.7079864610304\\
153	-40.7350492396635\\
154	-40.6405032241364\\
155	-40.3651494224422\\
156	-40.1504630705807\\
157	-39.5272836073848\\
158	-38.792267653329\\
159	-38.4272287460992\\
160	-38.9561853424272\\
161	-40.0974078951085\\
162	-40.1266722263973\\
163	-39.785689070857\\
164	-39.3904635518935\\
165	-39.4364553823933\\
166	-38.7675161819392\\
167	-38.9392219463423\\
168	-38.4464370548603\\
169	-37.4414093010701\\
170	-36.8384211722961\\
171	-37.763299139291\\
172	-37.9953742137359\\
173	-37.2637013325052\\
174	-37.2413400328124\\
175	-36.9997889800459\\
176	-37.0045095268116\\
177	-36.7014700875858\\
178	-36.4261339843527\\
179	-36.6205927259132\\
180	-37.6861166571578\\
181	-37.6211364131236\\
182	-37.9234369673119\\
183	-37.5037586079944\\
184	-37.582782578722\\
185	-37.1524975796374\\
186	-36.5394020603518\\
187	-36.4335351305984\\
188	-37.3211832814352\\
189	-37.2695783357305\\
190	-36.5987594916508\\
191	-36.9452518608838\\
192	-37.0575693476256\\
193	-37.0447842238401\\
194	-35.9571248887183\\
195	-35.7643377897755\\
196	-36.7204901514943\\
197	-36.4383174146219\\
198	-36.505762030719\\
199	-35.9666430800494\\
199	-35.9666430800494\\
199	-25\\
113	-25\\
113	-36.351475336133\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
113	-36.351475336133\\
114	-36.8479511671828\\
115	-37.0632116240475\\
116	-37.0661319571525\\
117	-37.2588816303491\\
118	-37.3990845639327\\
119	-37.5570851885126\\
120	-37.7057218158072\\
121	-37.5588812762327\\
122	-38.2536505185237\\
123	-38.5534615708318\\
124	-39.1976275498693\\
125	-39.4582077510982\\
126	-39.3643484163815\\
127	-39.9526374505114\\
128	-40.3569876273323\\
129	-39.4236330039063\\
130	-40.1975152983885\\
131	-40.1591960960801\\
132	-39.2141563845845\\
133	-39.6009047321718\\
134	-39.9876530797592\\
135	-40.5695678694775\\
136	-41.2810930139678\\
137	-40.7254448885807\\
138	-40.8653355994745\\
139	-40.517168397127\\
140	-41.1436300938016\\
141	-41.2916902925916\\
142	-41.100108632918\\
143	-41.0791236015771\\
144	-40.6120066609437\\
145	-39.7632521134971\\
146	-39.8505505835477\\
147	-40.1249030448183\\
148	-39.9158992879064\\
149	-39.5932387658054\\
150	-40.4875413625722\\
151	-40.3172237143515\\
152	-40.7079864610304\\
153	-40.7350492396635\\
154	-40.6405032241364\\
155	-40.3651494224422\\
156	-40.1504630705807\\
157	-39.5272836073848\\
158	-38.792267653329\\
159	-38.4272287460992\\
160	-38.9561853424272\\
161	-40.0974078951085\\
162	-40.1266722263973\\
163	-39.785689070857\\
164	-39.3904635518935\\
165	-39.4364553823933\\
166	-38.7675161819392\\
167	-38.9392219463423\\
168	-38.4464370548603\\
169	-37.4414093010701\\
170	-36.8384211722961\\
171	-37.763299139291\\
172	-37.9953742137359\\
173	-37.2637013325052\\
174	-37.2413400328124\\
175	-36.9997889800459\\
176	-37.0045095268116\\
177	-36.7014700875858\\
178	-36.4261339843527\\
179	-36.6205927259132\\
180	-37.6861166571578\\
181	-37.6211364131236\\
182	-37.9234369673119\\
183	-37.5037586079944\\
184	-37.582782578722\\
185	-37.1524975796374\\
186	-36.5394020603518\\
187	-36.4335351305984\\
188	-37.3211832814352\\
189	-37.2695783357305\\
190	-36.5987594916508\\
191	-36.9452518608838\\
192	-37.0575693476256\\
193	-37.0447842238401\\
194	-35.9571248887183\\
195	-35.7643377897755\\
196	-36.7204901514943\\
197	-36.4383174146219\\
198	-36.505762030719\\
199	-35.9666430800494\\
199	-35.9666430800494\\
199	-25\\
113	-25\\
113	-36.351475336133\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
113	-36.351475336133\\
114	-36.8479511671828\\
115	-37.0632116240475\\
116	-37.0661319571525\\
117	-37.2588816303491\\
118	-37.3990845639327\\
119	-37.5570851885126\\
120	-37.7057218158072\\
121	-37.5588812762327\\
122	-38.2536505185237\\
123	-38.5534615708318\\
124	-39.1976275498693\\
125	-39.4582077510982\\
126	-39.3643484163815\\
127	-39.9526374505114\\
128	-40.3569876273323\\
129	-39.4236330039063\\
130	-40.1975152983885\\
131	-40.1591960960801\\
132	-39.2141563845845\\
133	-39.6009047321718\\
134	-39.9876530797592\\
135	-40.5695678694775\\
136	-41.2810930139678\\
137	-40.7254448885807\\
138	-40.8653355994745\\
139	-40.517168397127\\
140	-41.1436300938016\\
141	-41.2916902925916\\
142	-41.100108632918\\
143	-41.0791236015771\\
144	-40.6120066609437\\
145	-39.7632521134971\\
146	-39.8505505835477\\
147	-40.1249030448183\\
148	-39.9158992879064\\
149	-39.5932387658054\\
150	-40.4875413625722\\
151	-40.3172237143515\\
152	-40.7079864610304\\
153	-40.7350492396635\\
154	-40.6405032241364\\
155	-40.3651494224422\\
156	-40.1504630705807\\
157	-39.5272836073848\\
158	-38.792267653329\\
159	-38.4272287460992\\
160	-38.9561853424272\\
161	-40.0974078951085\\
162	-40.1266722263973\\
163	-39.785689070857\\
164	-39.3904635518935\\
165	-39.4364553823933\\
166	-38.7675161819392\\
167	-38.9392219463423\\
168	-38.4464370548603\\
169	-37.4414093010701\\
170	-36.8384211722961\\
171	-37.763299139291\\
172	-37.9953742137359\\
173	-37.2637013325052\\
174	-37.2413400328124\\
175	-36.9997889800459\\
176	-37.0045095268116\\
177	-36.7014700875858\\
178	-36.4261339843527\\
179	-36.6205927259132\\
180	-37.6861166571578\\
181	-37.6211364131236\\
182	-37.9234369673119\\
183	-37.5037586079944\\
184	-37.582782578722\\
185	-37.1524975796374\\
186	-36.5394020603518\\
187	-36.4335351305984\\
188	-37.3211832814352\\
189	-37.2695783357305\\
190	-36.5987594916508\\
191	-36.9452518608838\\
192	-37.0575693476256\\
193	-37.0447842238401\\
194	-35.9571248887183\\
195	-35.7643377897755\\
196	-36.7204901514943\\
197	-36.4383174146219\\
198	-36.505762030719\\
199	-35.9666430800494\\
199	-35.9666430800494\\
199	-25\\
113	-25\\
113	-36.351475336133\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
115	-37.0632116240475\\
116	-37.0661319571525\\
117	-37.2588816303491\\
118	-37.3990845639327\\
119	-37.5570851885126\\
120	-37.7057218158072\\
121	-37.5588812762327\\
122	-38.2536505185237\\
123	-38.5534615708318\\
124	-39.1976275498693\\
125	-39.4582077510982\\
126	-39.3643484163815\\
127	-39.9526374505114\\
128	-40.3569876273323\\
129	-39.4236330039063\\
130	-40.1975152983885\\
131	-40.1591960960801\\
132	-39.2141563845845\\
133	-39.6009047321718\\
134	-39.9876530797592\\
135	-40.5695678694775\\
136	-41.2810930139678\\
137	-40.7254448885807\\
138	-40.8653355994745\\
139	-40.517168397127\\
140	-41.1436300938016\\
141	-41.2916902925916\\
142	-41.100108632918\\
143	-41.0791236015771\\
144	-40.6120066609437\\
145	-39.7632521134971\\
146	-39.8505505835477\\
147	-40.1249030448183\\
148	-39.9158992879064\\
149	-39.5932387658054\\
150	-40.4875413625722\\
151	-40.3172237143515\\
152	-40.7079864610304\\
153	-40.7350492396635\\
154	-40.6405032241364\\
155	-40.3651494224422\\
156	-40.1504630705807\\
157	-39.5272836073848\\
158	-38.792267653329\\
159	-38.4272287460992\\
160	-38.9561853424272\\
161	-40.0974078951085\\
162	-40.1266722263973\\
163	-39.785689070857\\
164	-39.3904635518935\\
165	-39.4364553823933\\
166	-38.7675161819392\\
167	-38.9392219463423\\
168	-38.4464370548603\\
169	-37.4414093010701\\
170	-36.8384211722961\\
171	-37.763299139291\\
172	-37.9953742137359\\
173	-37.2637013325052\\
174	-37.2413400328124\\
175	-36.9997889800459\\
176	-37.0045095268116\\
177	-36.7014700875858\\
178	-36.4261339843527\\
179	-36.6205927259132\\
180	-37.6861166571578\\
181	-37.6211364131236\\
182	-37.9234369673119\\
183	-37.5037586079944\\
184	-37.582782578722\\
185	-37.1524975796374\\
186	-36.5394020603518\\
187	-36.4335351305984\\
188	-37.3211832814352\\
189	-37.2695783357305\\
190	-36.5987594916508\\
191	-36.9452518608838\\
192	-37.0575693476256\\
193	-37.0447842238401\\
194	-35.9571248887183\\
195	-35.7643377897755\\
196	-36.7204901514943\\
197	-36.4383174146219\\
198	-36.505762030719\\
198	-36.505762030719\\
198	-25\\
115	-25\\
115	-37.0632116240475\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
115	-37.0632116240475\\
116	-37.0661319571525\\
117	-37.2588816303491\\
118	-37.3990845639327\\
119	-37.5570851885126\\
120	-37.7057218158072\\
121	-37.5588812762327\\
122	-38.2536505185237\\
123	-38.5534615708318\\
124	-39.1976275498693\\
125	-39.4582077510982\\
126	-39.3643484163815\\
127	-39.9526374505114\\
128	-40.3569876273323\\
129	-39.4236330039063\\
130	-40.1975152983885\\
131	-40.1591960960801\\
132	-39.2141563845845\\
133	-39.6009047321718\\
134	-39.9876530797592\\
135	-40.5695678694775\\
136	-41.2810930139678\\
137	-40.7254448885807\\
138	-40.8653355994745\\
139	-40.517168397127\\
140	-41.1436300938016\\
141	-41.2916902925916\\
142	-41.100108632918\\
143	-41.0791236015771\\
144	-40.6120066609437\\
145	-39.7632521134971\\
146	-39.8505505835477\\
147	-40.1249030448183\\
148	-39.9158992879064\\
149	-39.5932387658054\\
150	-40.4875413625722\\
151	-40.3172237143515\\
152	-40.7079864610304\\
153	-40.7350492396635\\
154	-40.6405032241364\\
155	-40.3651494224422\\
156	-40.1504630705807\\
157	-39.5272836073848\\
158	-38.792267653329\\
159	-38.4272287460992\\
160	-38.9561853424272\\
161	-40.0974078951085\\
162	-40.1266722263973\\
163	-39.785689070857\\
164	-39.3904635518935\\
165	-39.4364553823933\\
166	-38.7675161819392\\
167	-38.9392219463423\\
168	-38.4464370548603\\
169	-37.4414093010701\\
170	-36.8384211722961\\
171	-37.763299139291\\
172	-37.9953742137359\\
173	-37.2637013325052\\
174	-37.2413400328124\\
175	-36.9997889800459\\
176	-37.0045095268116\\
177	-36.7014700875858\\
178	-36.4261339843527\\
179	-36.6205927259132\\
180	-37.6861166571578\\
181	-37.6211364131236\\
182	-37.9234369673119\\
183	-37.5037586079944\\
184	-37.582782578722\\
185	-37.1524975796374\\
186	-36.5394020603518\\
187	-36.4335351305984\\
188	-37.3211832814352\\
189	-37.2695783357305\\
190	-36.5987594916508\\
191	-36.9452518608838\\
192	-37.0575693476256\\
193	-37.0447842238401\\
194	-35.9571248887183\\
195	-35.7643377897755\\
196	-36.7204901514943\\
197	-36.4383174146219\\
198	-36.505762030719\\
198	-36.505762030719\\
198	-25\\
115	-25\\
115	-37.0632116240475\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
115	-37.0632116240475\\
116	-37.0661319571525\\
117	-37.2588816303491\\
118	-37.3990845639327\\
119	-37.5570851885126\\
120	-37.7057218158072\\
121	-37.5588812762327\\
122	-38.2536505185237\\
123	-38.5534615708318\\
124	-39.1976275498693\\
125	-39.4582077510982\\
126	-39.3643484163815\\
127	-39.9526374505114\\
128	-40.3569876273323\\
129	-39.4236330039063\\
130	-40.1975152983885\\
131	-40.1591960960801\\
132	-39.2141563845845\\
133	-39.6009047321718\\
134	-39.9876530797592\\
135	-40.5695678694775\\
136	-41.2810930139678\\
137	-40.7254448885807\\
138	-40.8653355994745\\
139	-40.517168397127\\
140	-41.1436300938016\\
141	-41.2916902925916\\
142	-41.100108632918\\
143	-41.0791236015771\\
144	-40.6120066609437\\
145	-39.7632521134971\\
146	-39.8505505835477\\
147	-40.1249030448183\\
148	-39.9158992879064\\
149	-39.5932387658054\\
150	-40.4875413625722\\
151	-40.3172237143515\\
152	-40.7079864610304\\
153	-40.7350492396635\\
154	-40.6405032241364\\
155	-40.3651494224422\\
156	-40.1504630705807\\
157	-39.5272836073848\\
158	-38.792267653329\\
159	-38.4272287460992\\
160	-38.9561853424272\\
161	-40.0974078951085\\
162	-40.1266722263973\\
163	-39.785689070857\\
164	-39.3904635518935\\
165	-39.4364553823933\\
166	-38.7675161819392\\
167	-38.9392219463423\\
168	-38.4464370548603\\
169	-37.4414093010701\\
170	-36.8384211722961\\
171	-37.763299139291\\
172	-37.9953742137359\\
173	-37.2637013325052\\
174	-37.2413400328124\\
175	-36.9997889800459\\
176	-37.0045095268116\\
177	-36.7014700875858\\
178	-36.4261339843527\\
179	-36.6205927259132\\
180	-37.6861166571578\\
181	-37.6211364131236\\
182	-37.9234369673119\\
183	-37.5037586079944\\
184	-37.582782578722\\
185	-37.1524975796374\\
186	-36.5394020603518\\
187	-36.4335351305984\\
188	-37.3211832814352\\
189	-37.2695783357305\\
190	-36.5987594916508\\
191	-36.9452518608838\\
191	-36.9452518608838\\
191	-25\\
115	-25\\
115	-37.0632116240475\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
117	-37.2588816303491\\
118	-37.3990845639327\\
119	-37.5570851885126\\
120	-37.7057218158072\\
121	-37.5588812762327\\
122	-38.2536505185237\\
123	-38.5534615708318\\
124	-39.1976275498693\\
125	-39.4582077510982\\
126	-39.3643484163815\\
127	-39.9526374505114\\
128	-40.3569876273323\\
129	-39.4236330039063\\
130	-40.1975152983885\\
131	-40.1591960960801\\
132	-39.2141563845845\\
133	-39.6009047321718\\
134	-39.9876530797592\\
135	-40.5695678694775\\
136	-41.2810930139678\\
137	-40.7254448885807\\
138	-40.8653355994745\\
139	-40.517168397127\\
140	-41.1436300938016\\
141	-41.2916902925916\\
142	-41.100108632918\\
143	-41.0791236015771\\
144	-40.6120066609437\\
145	-39.7632521134971\\
146	-39.8505505835477\\
147	-40.1249030448183\\
148	-39.9158992879064\\
149	-39.5932387658054\\
150	-40.4875413625722\\
151	-40.3172237143515\\
152	-40.7079864610304\\
153	-40.7350492396635\\
154	-40.6405032241364\\
155	-40.3651494224422\\
156	-40.1504630705807\\
157	-39.5272836073848\\
158	-38.792267653329\\
159	-38.4272287460992\\
160	-38.9561853424272\\
161	-40.0974078951085\\
162	-40.1266722263973\\
163	-39.785689070857\\
164	-39.3904635518935\\
165	-39.4364553823933\\
166	-38.7675161819392\\
167	-38.9392219463423\\
168	-38.4464370548603\\
169	-37.4414093010701\\
170	-36.8384211722961\\
171	-37.763299139291\\
172	-37.9953742137359\\
173	-37.2637013325052\\
174	-37.2413400328124\\
175	-36.9997889800459\\
176	-37.0045095268116\\
177	-36.7014700875858\\
178	-36.4261339843527\\
179	-36.6205927259132\\
180	-37.6861166571578\\
181	-37.6211364131236\\
182	-37.9234369673119\\
183	-37.5037586079944\\
184	-37.582782578722\\
185	-37.1524975796374\\
186	-36.5394020603518\\
187	-36.4335351305984\\
188	-37.3211832814352\\
189	-37.2695783357305\\
190	-36.5987594916508\\
191	-36.9452518608838\\
191	-36.9452518608838\\
191	-25\\
117	-25\\
117	-37.2588816303491\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
117	-37.2588816303491\\
118	-37.3990845639327\\
119	-37.5570851885126\\
120	-37.7057218158072\\
121	-37.5588812762327\\
122	-38.2536505185237\\
123	-38.5534615708318\\
124	-39.1976275498693\\
125	-39.4582077510982\\
126	-39.3643484163815\\
127	-39.9526374505114\\
128	-40.3569876273323\\
129	-39.4236330039063\\
130	-40.1975152983885\\
131	-40.1591960960801\\
132	-39.2141563845845\\
133	-39.6009047321718\\
134	-39.9876530797592\\
135	-40.5695678694775\\
136	-41.2810930139678\\
137	-40.7254448885807\\
138	-40.8653355994745\\
139	-40.517168397127\\
140	-41.1436300938016\\
141	-41.2916902925916\\
142	-41.100108632918\\
143	-41.0791236015771\\
144	-40.6120066609437\\
145	-39.7632521134971\\
146	-39.8505505835477\\
147	-40.1249030448183\\
148	-39.9158992879064\\
149	-39.5932387658054\\
150	-40.4875413625722\\
151	-40.3172237143515\\
152	-40.7079864610304\\
153	-40.7350492396635\\
154	-40.6405032241364\\
155	-40.3651494224422\\
156	-40.1504630705807\\
157	-39.5272836073848\\
158	-38.792267653329\\
159	-38.4272287460992\\
160	-38.9561853424272\\
161	-40.0974078951085\\
162	-40.1266722263973\\
163	-39.785689070857\\
164	-39.3904635518935\\
165	-39.4364553823933\\
166	-38.7675161819392\\
167	-38.9392219463423\\
168	-38.4464370548603\\
169	-37.4414093010701\\
170	-36.8384211722961\\
171	-37.763299139291\\
172	-37.9953742137359\\
173	-37.2637013325052\\
174	-37.2413400328124\\
175	-36.9997889800459\\
176	-37.0045095268116\\
177	-36.7014700875858\\
178	-36.4261339843527\\
179	-36.6205927259132\\
180	-37.6861166571578\\
181	-37.6211364131236\\
182	-37.9234369673119\\
183	-37.5037586079944\\
184	-37.582782578722\\
185	-37.1524975796374\\
186	-36.5394020603518\\
187	-36.4335351305984\\
188	-37.3211832814352\\
189	-37.2695783357305\\
189	-37.2695783357305\\
189	-25\\
117	-25\\
117	-37.2588816303491\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
117	-37.2588816303491\\
118	-37.3990845639327\\
119	-37.5570851885126\\
120	-37.7057218158072\\
121	-37.5588812762327\\
122	-38.2536505185237\\
123	-38.5534615708318\\
124	-39.1976275498693\\
125	-39.4582077510982\\
126	-39.3643484163815\\
127	-39.9526374505114\\
128	-40.3569876273323\\
129	-39.4236330039063\\
130	-40.1975152983885\\
131	-40.1591960960801\\
132	-39.2141563845845\\
133	-39.6009047321718\\
134	-39.9876530797592\\
135	-40.5695678694775\\
136	-41.2810930139678\\
137	-40.7254448885807\\
138	-40.8653355994745\\
139	-40.517168397127\\
140	-41.1436300938016\\
141	-41.2916902925916\\
142	-41.100108632918\\
143	-41.0791236015771\\
144	-40.6120066609437\\
145	-39.7632521134971\\
146	-39.8505505835477\\
147	-40.1249030448183\\
148	-39.9158992879064\\
149	-39.5932387658054\\
150	-40.4875413625722\\
151	-40.3172237143515\\
152	-40.7079864610304\\
153	-40.7350492396635\\
154	-40.6405032241364\\
155	-40.3651494224422\\
156	-40.1504630705807\\
157	-39.5272836073848\\
158	-38.792267653329\\
159	-38.4272287460992\\
160	-38.9561853424272\\
161	-40.0974078951085\\
162	-40.1266722263973\\
163	-39.785689070857\\
164	-39.3904635518935\\
165	-39.4364553823933\\
166	-38.7675161819392\\
167	-38.9392219463423\\
168	-38.4464370548603\\
169	-37.4414093010701\\
170	-36.8384211722961\\
171	-37.763299139291\\
172	-37.9953742137359\\
173	-37.2637013325052\\
174	-37.2413400328124\\
175	-36.9997889800459\\
176	-37.0045095268116\\
177	-36.7014700875858\\
178	-36.4261339843527\\
179	-36.6205927259132\\
180	-37.6861166571578\\
181	-37.6211364131236\\
182	-37.9234369673119\\
183	-37.5037586079944\\
184	-37.582782578722\\
185	-37.1524975796374\\
186	-36.5394020603518\\
187	-36.4335351305984\\
188	-37.3211832814352\\
189	-37.2695783357305\\
189	-37.2695783357305\\
189	-25\\
117	-25\\
117	-37.2588816303491\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
120	-37.7057218158072\\
121	-37.5588812762327\\
122	-38.2536505185237\\
123	-38.5534615708318\\
124	-39.1976275498693\\
125	-39.4582077510982\\
126	-39.3643484163815\\
127	-39.9526374505114\\
128	-40.3569876273323\\
129	-39.4236330039063\\
130	-40.1975152983885\\
131	-40.1591960960801\\
132	-39.2141563845845\\
133	-39.6009047321718\\
134	-39.9876530797592\\
135	-40.5695678694775\\
136	-41.2810930139678\\
137	-40.7254448885807\\
138	-40.8653355994745\\
139	-40.517168397127\\
140	-41.1436300938016\\
141	-41.2916902925916\\
142	-41.100108632918\\
143	-41.0791236015771\\
144	-40.6120066609437\\
145	-39.7632521134971\\
146	-39.8505505835477\\
147	-40.1249030448183\\
148	-39.9158992879064\\
149	-39.5932387658054\\
150	-40.4875413625722\\
151	-40.3172237143515\\
152	-40.7079864610304\\
153	-40.7350492396635\\
154	-40.6405032241364\\
155	-40.3651494224422\\
156	-40.1504630705807\\
157	-39.5272836073848\\
158	-38.792267653329\\
159	-38.4272287460992\\
160	-38.9561853424272\\
161	-40.0974078951085\\
162	-40.1266722263973\\
163	-39.785689070857\\
164	-39.3904635518935\\
165	-39.4364553823933\\
166	-38.7675161819392\\
167	-38.9392219463423\\
168	-38.4464370548603\\
169	-37.4414093010701\\
170	-36.8384211722961\\
171	-37.763299139291\\
172	-37.9953742137359\\
173	-37.2637013325052\\
174	-37.2413400328124\\
175	-36.9997889800459\\
176	-37.0045095268116\\
177	-36.7014700875858\\
178	-36.4261339843527\\
179	-36.6205927259132\\
180	-37.6861166571578\\
181	-37.6211364131236\\
182	-37.9234369673119\\
183	-37.5037586079944\\
184	-37.582782578722\\
185	-37.1524975796374\\
186	-36.5394020603518\\
187	-36.4335351305984\\
188	-37.3211832814352\\
189	-37.2695783357305\\
189	-37.2695783357305\\
189	-25\\
120	-25\\
120	-37.7057218158072\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
120	-37.7057218158072\\
121	-37.5588812762327\\
122	-38.2536505185237\\
123	-38.5534615708318\\
124	-39.1976275498693\\
125	-39.4582077510982\\
126	-39.3643484163815\\
127	-39.9526374505114\\
128	-40.3569876273323\\
129	-39.4236330039063\\
130	-40.1975152983885\\
131	-40.1591960960801\\
132	-39.2141563845845\\
133	-39.6009047321718\\
134	-39.9876530797592\\
135	-40.5695678694775\\
136	-41.2810930139678\\
137	-40.7254448885807\\
138	-40.8653355994745\\
139	-40.517168397127\\
140	-41.1436300938016\\
141	-41.2916902925916\\
142	-41.100108632918\\
143	-41.0791236015771\\
144	-40.6120066609437\\
145	-39.7632521134971\\
146	-39.8505505835477\\
147	-40.1249030448183\\
148	-39.9158992879064\\
149	-39.5932387658054\\
150	-40.4875413625722\\
151	-40.3172237143515\\
152	-40.7079864610304\\
153	-40.7350492396635\\
154	-40.6405032241364\\
155	-40.3651494224422\\
156	-40.1504630705807\\
157	-39.5272836073848\\
158	-38.792267653329\\
159	-38.4272287460992\\
160	-38.9561853424272\\
161	-40.0974078951085\\
162	-40.1266722263973\\
163	-39.785689070857\\
164	-39.3904635518935\\
165	-39.4364553823933\\
166	-38.7675161819392\\
167	-38.9392219463423\\
168	-38.4464370548603\\
169	-37.4414093010701\\
170	-36.8384211722961\\
171	-37.763299139291\\
172	-37.9953742137359\\
173	-37.2637013325052\\
174	-37.2413400328124\\
175	-36.9997889800459\\
176	-37.0045095268116\\
177	-36.7014700875858\\
178	-36.4261339843527\\
179	-36.6205927259132\\
180	-37.6861166571578\\
181	-37.6211364131236\\
182	-37.9234369673119\\
183	-37.5037586079944\\
184	-37.582782578722\\
185	-37.1524975796374\\
186	-36.5394020603518\\
187	-36.4335351305984\\
188	-37.3211832814352\\
189	-37.2695783357305\\
189	-37.2695783357305\\
189	-25\\
120	-25\\
120	-37.7057218158072\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
120	-37.7057218158072\\
121	-37.5588812762327\\
122	-38.2536505185237\\
123	-38.5534615708318\\
124	-39.1976275498693\\
125	-39.4582077510982\\
126	-39.3643484163815\\
127	-39.9526374505114\\
128	-40.3569876273323\\
129	-39.4236330039063\\
130	-40.1975152983885\\
131	-40.1591960960801\\
132	-39.2141563845845\\
133	-39.6009047321718\\
134	-39.9876530797592\\
135	-40.5695678694775\\
136	-41.2810930139678\\
137	-40.7254448885807\\
138	-40.8653355994745\\
139	-40.517168397127\\
140	-41.1436300938016\\
141	-41.2916902925916\\
142	-41.100108632918\\
143	-41.0791236015771\\
144	-40.6120066609437\\
145	-39.7632521134971\\
146	-39.8505505835477\\
147	-40.1249030448183\\
148	-39.9158992879064\\
149	-39.5932387658054\\
150	-40.4875413625722\\
151	-40.3172237143515\\
152	-40.7079864610304\\
153	-40.7350492396635\\
154	-40.6405032241364\\
155	-40.3651494224422\\
156	-40.1504630705807\\
157	-39.5272836073848\\
158	-38.792267653329\\
159	-38.4272287460992\\
160	-38.9561853424272\\
161	-40.0974078951085\\
162	-40.1266722263973\\
163	-39.785689070857\\
164	-39.3904635518935\\
165	-39.4364553823933\\
166	-38.7675161819392\\
167	-38.9392219463423\\
168	-38.4464370548603\\
169	-37.4414093010701\\
170	-36.8384211722961\\
171	-37.763299139291\\
172	-37.9953742137359\\
173	-37.2637013325052\\
174	-37.2413400328124\\
175	-36.9997889800459\\
176	-37.0045095268116\\
177	-36.7014700875858\\
178	-36.4261339843527\\
179	-36.6205927259132\\
180	-37.6861166571578\\
181	-37.6211364131236\\
182	-37.9234369673119\\
183	-37.5037586079944\\
184	-37.582782578722\\
185	-37.1524975796374\\
186	-36.5394020603518\\
187	-36.4335351305984\\
188	-37.3211832814352\\
189	-37.2695783357305\\
189	-37.2695783357305\\
189	-25\\
120	-25\\
120	-37.7057218158072\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
111	-65.3896626098395\\
112	-65.9151443739689\\
113	-66.1741876665287\\
114	-66.6706634975785\\
115	-66.8859239544432\\
116	-66.8888442875482\\
117	-67.0815939607448\\
118	-67.2217968943284\\
119	-67.3797975189083\\
120	-67.5284341462029\\
121	-67.3815936066283\\
122	-68.0763628489194\\
123	-68.3761739012275\\
124	-69.0203398802649\\
125	-69.2809200814939\\
126	-69.1870607467771\\
127	-69.775349780907\\
128	-70.1796999577279\\
129	-69.246345334302\\
130	-70.0202276287842\\
131	-69.9819084264758\\
132	-69.0368687149802\\
133	-69.4236170625675\\
134	-69.8103654101549\\
135	-70.3922801998731\\
136	-71.1038053443635\\
137	-70.5481572189764\\
138	-70.6880479298702\\
139	-70.3398807275227\\
140	-70.9663424241973\\
141	-71.1144026229873\\
142	-70.9228209633137\\
143	-70.9018359319728\\
144	-70.4347189913394\\
145	-69.5859644438928\\
146	-69.6732629139434\\
147	-69.9476153752139\\
148	-69.7386116183021\\
149	-69.4159510962011\\
150	-70.3102536929679\\
151	-70.1399360447471\\
152	-70.5306987914261\\
153	-70.5577615700592\\
154	-70.4632155545321\\
155	-70.1878617528379\\
156	-69.9731754009764\\
157	-69.3499959377805\\
158	-68.6149799837247\\
159	-68.2499410764949\\
160	-68.7788976728229\\
161	-69.9201202255042\\
162	-69.949384556793\\
163	-69.6084014012527\\
164	-69.2131758822892\\
165	-69.259167712789\\
166	-68.5902285123349\\
167	-68.761934276738\\
168	-68.269149385256\\
169	-67.2641216314658\\
170	-66.6611335026917\\
171	-67.5860114696867\\
172	-67.8180865441316\\
173	-67.0864136629009\\
174	-67.0640523632081\\
175	-66.8225013104416\\
176	-66.8272218572073\\
177	-66.5241824179815\\
178	-66.2488463147484\\
179	-66.4433050563089\\
180	-67.5088289875535\\
181	-67.4438487435193\\
182	-67.7461492977076\\
183	-67.3264709383901\\
184	-67.4054949091177\\
185	-66.9752099100331\\
186	-66.3621143907475\\
187	-66.2562474609941\\
188	-67.1438956118309\\
189	-67.0922906661262\\
190	-66.4214718220465\\
191	-66.7679641912795\\
192	-66.8802816780212\\
193	-66.8674965542358\\
194	-65.779837219114\\
195	-65.5870501201712\\
196	-66.54320248189\\
197	-66.2610297450176\\
198	-66.3284743611147\\
199	-65.7893554104451\\
199	-65.7893554104451\\
199	-72\\
111	-72\\
111	-65.3896626098395\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
111	-65.3896626098395\\
112	-65.9151443739689\\
113	-66.1741876665287\\
114	-66.6706634975785\\
115	-66.8859239544432\\
116	-66.8888442875482\\
117	-67.0815939607448\\
118	-67.2217968943284\\
119	-67.3797975189083\\
120	-67.5284341462029\\
121	-67.3815936066283\\
122	-68.0763628489194\\
123	-68.3761739012275\\
124	-69.0203398802649\\
125	-69.2809200814939\\
126	-69.1870607467771\\
127	-69.775349780907\\
128	-70.1796999577279\\
129	-69.246345334302\\
130	-70.0202276287842\\
131	-69.9819084264758\\
132	-69.0368687149802\\
133	-69.4236170625675\\
134	-69.8103654101549\\
135	-70.3922801998731\\
136	-71.1038053443635\\
137	-70.5481572189764\\
138	-70.6880479298702\\
139	-70.3398807275227\\
140	-70.9663424241973\\
141	-71.1144026229873\\
142	-70.9228209633137\\
143	-70.9018359319728\\
144	-70.4347189913394\\
145	-69.5859644438928\\
146	-69.6732629139434\\
147	-69.9476153752139\\
148	-69.7386116183021\\
149	-69.4159510962011\\
150	-70.3102536929679\\
151	-70.1399360447471\\
152	-70.5306987914261\\
153	-70.5577615700592\\
154	-70.4632155545321\\
155	-70.1878617528379\\
156	-69.9731754009764\\
157	-69.3499959377805\\
158	-68.6149799837247\\
159	-68.2499410764949\\
160	-68.7788976728229\\
161	-69.9201202255042\\
162	-69.949384556793\\
163	-69.6084014012527\\
164	-69.2131758822892\\
165	-69.259167712789\\
166	-68.5902285123349\\
167	-68.761934276738\\
168	-68.269149385256\\
169	-67.2641216314658\\
170	-66.6611335026917\\
171	-67.5860114696867\\
172	-67.8180865441316\\
173	-67.0864136629009\\
174	-67.0640523632081\\
175	-66.8225013104416\\
176	-66.8272218572073\\
177	-66.5241824179815\\
178	-66.2488463147484\\
179	-66.4433050563089\\
180	-67.5088289875535\\
181	-67.4438487435193\\
182	-67.7461492977076\\
183	-67.3264709383901\\
184	-67.4054949091177\\
185	-66.9752099100331\\
186	-66.3621143907475\\
187	-66.2562474609941\\
188	-67.1438956118309\\
189	-67.0922906661262\\
190	-66.4214718220465\\
191	-66.7679641912795\\
192	-66.8802816780212\\
193	-66.8674965542358\\
194	-65.779837219114\\
195	-65.5870501201712\\
196	-66.54320248189\\
197	-66.2610297450176\\
198	-66.3284743611147\\
199	-65.7893554104451\\
199	-65.7893554104451\\
199	-72\\
111	-72\\
111	-65.3896626098395\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
111	-65.3896626098395\\
112	-65.9151443739689\\
113	-66.1741876665287\\
114	-66.6706634975785\\
115	-66.8859239544432\\
116	-66.8888442875482\\
117	-67.0815939607448\\
118	-67.2217968943284\\
119	-67.3797975189083\\
120	-67.5284341462029\\
121	-67.3815936066283\\
122	-68.0763628489194\\
123	-68.3761739012275\\
124	-69.0203398802649\\
125	-69.2809200814939\\
126	-69.1870607467771\\
127	-69.775349780907\\
128	-70.1796999577279\\
129	-69.246345334302\\
130	-70.0202276287842\\
131	-69.9819084264758\\
132	-69.0368687149802\\
133	-69.4236170625675\\
134	-69.8103654101549\\
135	-70.3922801998731\\
136	-71.1038053443635\\
137	-70.5481572189764\\
138	-70.6880479298702\\
139	-70.3398807275227\\
140	-70.9663424241973\\
141	-71.1144026229873\\
142	-70.9228209633137\\
143	-70.9018359319728\\
144	-70.4347189913394\\
145	-69.5859644438928\\
146	-69.6732629139434\\
147	-69.9476153752139\\
148	-69.7386116183021\\
149	-69.4159510962011\\
150	-70.3102536929679\\
151	-70.1399360447471\\
152	-70.5306987914261\\
153	-70.5577615700592\\
154	-70.4632155545321\\
155	-70.1878617528379\\
156	-69.9731754009764\\
157	-69.3499959377805\\
158	-68.6149799837247\\
159	-68.2499410764949\\
160	-68.7788976728229\\
161	-69.9201202255042\\
162	-69.949384556793\\
163	-69.6084014012527\\
164	-69.2131758822892\\
165	-69.259167712789\\
166	-68.5902285123349\\
167	-68.761934276738\\
168	-68.269149385256\\
169	-67.2641216314658\\
170	-66.6611335026917\\
171	-67.5860114696867\\
172	-67.8180865441316\\
173	-67.0864136629009\\
174	-67.0640523632081\\
175	-66.8225013104416\\
176	-66.8272218572073\\
177	-66.5241824179815\\
178	-66.2488463147484\\
179	-66.4433050563089\\
180	-67.5088289875535\\
181	-67.4438487435193\\
182	-67.7461492977076\\
183	-67.3264709383901\\
184	-67.4054949091177\\
185	-66.9752099100331\\
186	-66.3621143907475\\
187	-66.2562474609941\\
188	-67.1438956118309\\
189	-67.0922906661262\\
190	-66.4214718220465\\
191	-66.7679641912795\\
192	-66.8802816780212\\
193	-66.8674965542358\\
194	-65.779837219114\\
195	-65.5870501201712\\
196	-66.54320248189\\
197	-66.2610297450176\\
198	-66.3284743611147\\
199	-65.7893554104451\\
199	-65.7893554104451\\
199	-72\\
111	-72\\
111	-65.3896626098395\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
113	-66.1741876665287\\
114	-66.6706634975785\\
115	-66.8859239544432\\
116	-66.8888442875482\\
117	-67.0815939607448\\
118	-67.2217968943284\\
119	-67.3797975189083\\
120	-67.5284341462029\\
121	-67.3815936066283\\
122	-68.0763628489194\\
123	-68.3761739012275\\
124	-69.0203398802649\\
125	-69.2809200814939\\
126	-69.1870607467771\\
127	-69.775349780907\\
128	-70.1796999577279\\
129	-69.246345334302\\
130	-70.0202276287842\\
131	-69.9819084264758\\
132	-69.0368687149802\\
133	-69.4236170625675\\
134	-69.8103654101549\\
135	-70.3922801998731\\
136	-71.1038053443635\\
137	-70.5481572189764\\
138	-70.6880479298702\\
139	-70.3398807275227\\
140	-70.9663424241973\\
141	-71.1144026229873\\
142	-70.9228209633137\\
143	-70.9018359319728\\
144	-70.4347189913394\\
145	-69.5859644438928\\
146	-69.6732629139434\\
147	-69.9476153752139\\
148	-69.7386116183021\\
149	-69.4159510962011\\
150	-70.3102536929679\\
151	-70.1399360447471\\
152	-70.5306987914261\\
153	-70.5577615700592\\
154	-70.4632155545321\\
155	-70.1878617528379\\
156	-69.9731754009764\\
157	-69.3499959377805\\
158	-68.6149799837247\\
159	-68.2499410764949\\
160	-68.7788976728229\\
161	-69.9201202255042\\
162	-69.949384556793\\
163	-69.6084014012527\\
164	-69.2131758822892\\
165	-69.259167712789\\
166	-68.5902285123349\\
167	-68.761934276738\\
168	-68.269149385256\\
169	-67.2641216314658\\
170	-66.6611335026917\\
171	-67.5860114696867\\
172	-67.8180865441316\\
173	-67.0864136629009\\
174	-67.0640523632081\\
175	-66.8225013104416\\
176	-66.8272218572073\\
177	-66.5241824179815\\
178	-66.2488463147484\\
179	-66.4433050563089\\
180	-67.5088289875535\\
181	-67.4438487435193\\
182	-67.7461492977076\\
183	-67.3264709383901\\
184	-67.4054949091177\\
185	-66.9752099100331\\
186	-66.3621143907475\\
187	-66.2562474609941\\
188	-67.1438956118309\\
189	-67.0922906661262\\
190	-66.4214718220465\\
191	-66.7679641912795\\
192	-66.8802816780212\\
193	-66.8674965542358\\
194	-65.779837219114\\
195	-65.5870501201712\\
196	-66.54320248189\\
197	-66.2610297450176\\
198	-66.3284743611147\\
199	-65.7893554104451\\
199	-65.7893554104451\\
199	-72\\
113	-72\\
113	-66.1741876665287\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
113	-66.1741876665287\\
114	-66.6706634975785\\
115	-66.8859239544432\\
116	-66.8888442875482\\
117	-67.0815939607448\\
118	-67.2217968943284\\
119	-67.3797975189083\\
120	-67.5284341462029\\
121	-67.3815936066283\\
122	-68.0763628489194\\
123	-68.3761739012275\\
124	-69.0203398802649\\
125	-69.2809200814939\\
126	-69.1870607467771\\
127	-69.775349780907\\
128	-70.1796999577279\\
129	-69.246345334302\\
130	-70.0202276287842\\
131	-69.9819084264758\\
132	-69.0368687149802\\
133	-69.4236170625675\\
134	-69.8103654101549\\
135	-70.3922801998731\\
136	-71.1038053443635\\
137	-70.5481572189764\\
138	-70.6880479298702\\
139	-70.3398807275227\\
140	-70.9663424241973\\
141	-71.1144026229873\\
142	-70.9228209633137\\
143	-70.9018359319728\\
144	-70.4347189913394\\
145	-69.5859644438928\\
146	-69.6732629139434\\
147	-69.9476153752139\\
148	-69.7386116183021\\
149	-69.4159510962011\\
150	-70.3102536929679\\
151	-70.1399360447471\\
152	-70.5306987914261\\
153	-70.5577615700592\\
154	-70.4632155545321\\
155	-70.1878617528379\\
156	-69.9731754009764\\
157	-69.3499959377805\\
158	-68.6149799837247\\
159	-68.2499410764949\\
160	-68.7788976728229\\
161	-69.9201202255042\\
162	-69.949384556793\\
163	-69.6084014012527\\
164	-69.2131758822892\\
165	-69.259167712789\\
166	-68.5902285123349\\
167	-68.761934276738\\
168	-68.269149385256\\
169	-67.2641216314658\\
170	-66.6611335026917\\
171	-67.5860114696867\\
172	-67.8180865441316\\
173	-67.0864136629009\\
174	-67.0640523632081\\
175	-66.8225013104416\\
176	-66.8272218572073\\
177	-66.5241824179815\\
178	-66.2488463147484\\
179	-66.4433050563089\\
180	-67.5088289875535\\
181	-67.4438487435193\\
182	-67.7461492977076\\
183	-67.3264709383901\\
184	-67.4054949091177\\
185	-66.9752099100331\\
186	-66.3621143907475\\
187	-66.2562474609941\\
188	-67.1438956118309\\
189	-67.0922906661262\\
190	-66.4214718220465\\
191	-66.7679641912795\\
192	-66.8802816780212\\
193	-66.8674965542358\\
194	-65.779837219114\\
195	-65.5870501201712\\
196	-66.54320248189\\
197	-66.2610297450176\\
198	-66.3284743611147\\
199	-65.7893554104451\\
199	-65.7893554104451\\
199	-72\\
113	-72\\
113	-66.1741876665287\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
113	-66.1741876665287\\
114	-66.6706634975785\\
115	-66.8859239544432\\
116	-66.8888442875482\\
117	-67.0815939607448\\
118	-67.2217968943284\\
119	-67.3797975189083\\
120	-67.5284341462029\\
121	-67.3815936066283\\
122	-68.0763628489194\\
123	-68.3761739012275\\
124	-69.0203398802649\\
125	-69.2809200814939\\
126	-69.1870607467771\\
127	-69.775349780907\\
128	-70.1796999577279\\
129	-69.246345334302\\
130	-70.0202276287842\\
131	-69.9819084264758\\
132	-69.0368687149802\\
133	-69.4236170625675\\
134	-69.8103654101549\\
135	-70.3922801998731\\
136	-71.1038053443635\\
137	-70.5481572189764\\
138	-70.6880479298702\\
139	-70.3398807275227\\
140	-70.9663424241973\\
141	-71.1144026229873\\
142	-70.9228209633137\\
143	-70.9018359319728\\
144	-70.4347189913394\\
145	-69.5859644438928\\
146	-69.6732629139434\\
147	-69.9476153752139\\
148	-69.7386116183021\\
149	-69.4159510962011\\
150	-70.3102536929679\\
151	-70.1399360447471\\
152	-70.5306987914261\\
153	-70.5577615700592\\
154	-70.4632155545321\\
155	-70.1878617528379\\
156	-69.9731754009764\\
157	-69.3499959377805\\
158	-68.6149799837247\\
159	-68.2499410764949\\
160	-68.7788976728229\\
161	-69.9201202255042\\
162	-69.949384556793\\
163	-69.6084014012527\\
164	-69.2131758822892\\
165	-69.259167712789\\
166	-68.5902285123349\\
167	-68.761934276738\\
168	-68.269149385256\\
169	-67.2641216314658\\
170	-66.6611335026917\\
171	-67.5860114696867\\
172	-67.8180865441316\\
173	-67.0864136629009\\
174	-67.0640523632081\\
175	-66.8225013104416\\
176	-66.8272218572073\\
177	-66.5241824179815\\
178	-66.2488463147484\\
179	-66.4433050563089\\
180	-67.5088289875535\\
181	-67.4438487435193\\
182	-67.7461492977076\\
183	-67.3264709383901\\
184	-67.4054949091177\\
185	-66.9752099100331\\
186	-66.3621143907475\\
187	-66.2562474609941\\
188	-67.1438956118309\\
189	-67.0922906661262\\
190	-66.4214718220465\\
191	-66.7679641912795\\
192	-66.8802816780212\\
193	-66.8674965542358\\
194	-65.779837219114\\
195	-65.5870501201712\\
196	-66.54320248189\\
197	-66.2610297450176\\
198	-66.3284743611147\\
199	-65.7893554104451\\
199	-65.7893554104451\\
199	-72\\
113	-72\\
113	-66.1741876665287\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
115	-66.8859239544432\\
116	-66.8888442875482\\
117	-67.0815939607448\\
118	-67.2217968943284\\
119	-67.3797975189083\\
120	-67.5284341462029\\
121	-67.3815936066283\\
122	-68.0763628489194\\
123	-68.3761739012275\\
124	-69.0203398802649\\
125	-69.2809200814939\\
126	-69.1870607467771\\
127	-69.775349780907\\
128	-70.1796999577279\\
129	-69.246345334302\\
130	-70.0202276287842\\
131	-69.9819084264758\\
132	-69.0368687149802\\
133	-69.4236170625675\\
134	-69.8103654101549\\
135	-70.3922801998731\\
136	-71.1038053443635\\
137	-70.5481572189764\\
138	-70.6880479298702\\
139	-70.3398807275227\\
140	-70.9663424241973\\
141	-71.1144026229873\\
142	-70.9228209633137\\
143	-70.9018359319728\\
144	-70.4347189913394\\
145	-69.5859644438928\\
146	-69.6732629139434\\
147	-69.9476153752139\\
148	-69.7386116183021\\
149	-69.4159510962011\\
150	-70.3102536929679\\
151	-70.1399360447471\\
152	-70.5306987914261\\
153	-70.5577615700592\\
154	-70.4632155545321\\
155	-70.1878617528379\\
156	-69.9731754009764\\
157	-69.3499959377805\\
158	-68.6149799837247\\
159	-68.2499410764949\\
160	-68.7788976728229\\
161	-69.9201202255042\\
162	-69.949384556793\\
163	-69.6084014012527\\
164	-69.2131758822892\\
165	-69.259167712789\\
166	-68.5902285123349\\
167	-68.761934276738\\
168	-68.269149385256\\
169	-67.2641216314658\\
170	-66.6611335026917\\
171	-67.5860114696867\\
172	-67.8180865441316\\
173	-67.0864136629009\\
174	-67.0640523632081\\
175	-66.8225013104416\\
176	-66.8272218572073\\
177	-66.5241824179815\\
178	-66.2488463147484\\
179	-66.4433050563089\\
180	-67.5088289875535\\
181	-67.4438487435193\\
182	-67.7461492977076\\
183	-67.3264709383901\\
184	-67.4054949091177\\
185	-66.9752099100331\\
186	-66.3621143907475\\
187	-66.2562474609941\\
188	-67.1438956118309\\
189	-67.0922906661262\\
190	-66.4214718220465\\
191	-66.7679641912795\\
192	-66.8802816780212\\
193	-66.8674965542358\\
194	-65.779837219114\\
195	-65.5870501201712\\
196	-66.54320248189\\
197	-66.2610297450176\\
198	-66.3284743611147\\
198	-66.3284743611147\\
198	-72\\
115	-72\\
115	-66.8859239544432\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
115	-66.8859239544432\\
116	-66.8888442875482\\
117	-67.0815939607448\\
118	-67.2217968943284\\
119	-67.3797975189083\\
120	-67.5284341462029\\
121	-67.3815936066283\\
122	-68.0763628489194\\
123	-68.3761739012275\\
124	-69.0203398802649\\
125	-69.2809200814939\\
126	-69.1870607467771\\
127	-69.775349780907\\
128	-70.1796999577279\\
129	-69.246345334302\\
130	-70.0202276287842\\
131	-69.9819084264758\\
132	-69.0368687149802\\
133	-69.4236170625675\\
134	-69.8103654101549\\
135	-70.3922801998731\\
136	-71.1038053443635\\
137	-70.5481572189764\\
138	-70.6880479298702\\
139	-70.3398807275227\\
140	-70.9663424241973\\
141	-71.1144026229873\\
142	-70.9228209633137\\
143	-70.9018359319728\\
144	-70.4347189913394\\
145	-69.5859644438928\\
146	-69.6732629139434\\
147	-69.9476153752139\\
148	-69.7386116183021\\
149	-69.4159510962011\\
150	-70.3102536929679\\
151	-70.1399360447471\\
152	-70.5306987914261\\
153	-70.5577615700592\\
154	-70.4632155545321\\
155	-70.1878617528379\\
156	-69.9731754009764\\
157	-69.3499959377805\\
158	-68.6149799837247\\
159	-68.2499410764949\\
160	-68.7788976728229\\
161	-69.9201202255042\\
162	-69.949384556793\\
163	-69.6084014012527\\
164	-69.2131758822892\\
165	-69.259167712789\\
166	-68.5902285123349\\
167	-68.761934276738\\
168	-68.269149385256\\
169	-67.2641216314658\\
170	-66.6611335026917\\
171	-67.5860114696867\\
172	-67.8180865441316\\
173	-67.0864136629009\\
174	-67.0640523632081\\
175	-66.8225013104416\\
176	-66.8272218572073\\
177	-66.5241824179815\\
178	-66.2488463147484\\
179	-66.4433050563089\\
180	-67.5088289875535\\
181	-67.4438487435193\\
182	-67.7461492977076\\
183	-67.3264709383901\\
184	-67.4054949091177\\
185	-66.9752099100331\\
186	-66.3621143907475\\
187	-66.2562474609941\\
188	-67.1438956118309\\
189	-67.0922906661262\\
190	-66.4214718220465\\
191	-66.7679641912795\\
192	-66.8802816780212\\
193	-66.8674965542358\\
194	-65.779837219114\\
195	-65.5870501201712\\
196	-66.54320248189\\
197	-66.2610297450176\\
198	-66.3284743611147\\
198	-66.3284743611147\\
198	-72\\
115	-72\\
115	-66.8859239544432\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
115	-66.8859239544432\\
116	-66.8888442875482\\
117	-67.0815939607448\\
118	-67.2217968943284\\
119	-67.3797975189083\\
120	-67.5284341462029\\
121	-67.3815936066283\\
122	-68.0763628489194\\
123	-68.3761739012275\\
124	-69.0203398802649\\
125	-69.2809200814939\\
126	-69.1870607467771\\
127	-69.775349780907\\
128	-70.1796999577279\\
129	-69.246345334302\\
130	-70.0202276287842\\
131	-69.9819084264758\\
132	-69.0368687149802\\
133	-69.4236170625675\\
134	-69.8103654101549\\
135	-70.3922801998731\\
136	-71.1038053443635\\
137	-70.5481572189764\\
138	-70.6880479298702\\
139	-70.3398807275227\\
140	-70.9663424241973\\
141	-71.1144026229873\\
142	-70.9228209633137\\
143	-70.9018359319728\\
144	-70.4347189913394\\
145	-69.5859644438928\\
146	-69.6732629139434\\
147	-69.9476153752139\\
148	-69.7386116183021\\
149	-69.4159510962011\\
150	-70.3102536929679\\
151	-70.1399360447471\\
152	-70.5306987914261\\
153	-70.5577615700592\\
154	-70.4632155545321\\
155	-70.1878617528379\\
156	-69.9731754009764\\
157	-69.3499959377805\\
158	-68.6149799837247\\
159	-68.2499410764949\\
160	-68.7788976728229\\
161	-69.9201202255042\\
162	-69.949384556793\\
163	-69.6084014012527\\
164	-69.2131758822892\\
165	-69.259167712789\\
166	-68.5902285123349\\
167	-68.761934276738\\
168	-68.269149385256\\
169	-67.2641216314658\\
170	-66.6611335026917\\
171	-67.5860114696867\\
172	-67.8180865441316\\
173	-67.0864136629009\\
174	-67.0640523632081\\
175	-66.8225013104416\\
176	-66.8272218572073\\
177	-66.5241824179815\\
178	-66.2488463147484\\
179	-66.4433050563089\\
180	-67.5088289875535\\
181	-67.4438487435193\\
182	-67.7461492977076\\
183	-67.3264709383901\\
184	-67.4054949091177\\
185	-66.9752099100331\\
186	-66.3621143907475\\
187	-66.2562474609941\\
188	-67.1438956118309\\
189	-67.0922906661262\\
190	-66.4214718220465\\
191	-66.7679641912795\\
191	-66.7679641912795\\
191	-72\\
115	-72\\
115	-66.8859239544432\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
117	-67.0815939607448\\
118	-67.2217968943284\\
119	-67.3797975189083\\
120	-67.5284341462029\\
121	-67.3815936066283\\
122	-68.0763628489194\\
123	-68.3761739012275\\
124	-69.0203398802649\\
125	-69.2809200814939\\
126	-69.1870607467771\\
127	-69.775349780907\\
128	-70.1796999577279\\
129	-69.246345334302\\
130	-70.0202276287842\\
131	-69.9819084264758\\
132	-69.0368687149802\\
133	-69.4236170625675\\
134	-69.8103654101549\\
135	-70.3922801998731\\
136	-71.1038053443635\\
137	-70.5481572189764\\
138	-70.6880479298702\\
139	-70.3398807275227\\
140	-70.9663424241973\\
141	-71.1144026229873\\
142	-70.9228209633137\\
143	-70.9018359319728\\
144	-70.4347189913394\\
145	-69.5859644438928\\
146	-69.6732629139434\\
147	-69.9476153752139\\
148	-69.7386116183021\\
149	-69.4159510962011\\
150	-70.3102536929679\\
151	-70.1399360447471\\
152	-70.5306987914261\\
153	-70.5577615700592\\
154	-70.4632155545321\\
155	-70.1878617528379\\
156	-69.9731754009764\\
157	-69.3499959377805\\
158	-68.6149799837247\\
159	-68.2499410764949\\
160	-68.7788976728229\\
161	-69.9201202255042\\
162	-69.949384556793\\
163	-69.6084014012527\\
164	-69.2131758822892\\
165	-69.259167712789\\
166	-68.5902285123349\\
167	-68.761934276738\\
168	-68.269149385256\\
169	-67.2641216314658\\
170	-66.6611335026917\\
171	-67.5860114696867\\
172	-67.8180865441316\\
173	-67.0864136629009\\
174	-67.0640523632081\\
175	-66.8225013104416\\
176	-66.8272218572073\\
177	-66.5241824179815\\
178	-66.2488463147484\\
179	-66.4433050563089\\
180	-67.5088289875535\\
181	-67.4438487435193\\
182	-67.7461492977076\\
183	-67.3264709383901\\
184	-67.4054949091177\\
185	-66.9752099100331\\
186	-66.3621143907475\\
187	-66.2562474609941\\
188	-67.1438956118309\\
189	-67.0922906661262\\
190	-66.4214718220465\\
191	-66.7679641912795\\
191	-66.7679641912795\\
191	-72\\
117	-72\\
117	-67.0815939607448\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
117	-67.0815939607448\\
118	-67.2217968943284\\
119	-67.3797975189083\\
120	-67.5284341462029\\
121	-67.3815936066283\\
122	-68.0763628489194\\
123	-68.3761739012275\\
124	-69.0203398802649\\
125	-69.2809200814939\\
126	-69.1870607467771\\
127	-69.775349780907\\
128	-70.1796999577279\\
129	-69.246345334302\\
130	-70.0202276287842\\
131	-69.9819084264758\\
132	-69.0368687149802\\
133	-69.4236170625675\\
134	-69.8103654101549\\
135	-70.3922801998731\\
136	-71.1038053443635\\
137	-70.5481572189764\\
138	-70.6880479298702\\
139	-70.3398807275227\\
140	-70.9663424241973\\
141	-71.1144026229873\\
142	-70.9228209633137\\
143	-70.9018359319728\\
144	-70.4347189913394\\
145	-69.5859644438928\\
146	-69.6732629139434\\
147	-69.9476153752139\\
148	-69.7386116183021\\
149	-69.4159510962011\\
150	-70.3102536929679\\
151	-70.1399360447471\\
152	-70.5306987914261\\
153	-70.5577615700592\\
154	-70.4632155545321\\
155	-70.1878617528379\\
156	-69.9731754009764\\
157	-69.3499959377805\\
158	-68.6149799837247\\
159	-68.2499410764949\\
160	-68.7788976728229\\
161	-69.9201202255042\\
162	-69.949384556793\\
163	-69.6084014012527\\
164	-69.2131758822892\\
165	-69.259167712789\\
166	-68.5902285123349\\
167	-68.761934276738\\
168	-68.269149385256\\
169	-67.2641216314658\\
170	-66.6611335026917\\
171	-67.5860114696867\\
172	-67.8180865441316\\
173	-67.0864136629009\\
174	-67.0640523632081\\
175	-66.8225013104416\\
176	-66.8272218572073\\
177	-66.5241824179815\\
178	-66.2488463147484\\
179	-66.4433050563089\\
180	-67.5088289875535\\
181	-67.4438487435193\\
182	-67.7461492977076\\
183	-67.3264709383901\\
184	-67.4054949091177\\
185	-66.9752099100331\\
186	-66.3621143907475\\
187	-66.2562474609941\\
188	-67.1438956118309\\
189	-67.0922906661262\\
189	-67.0922906661262\\
189	-72\\
117	-72\\
117	-67.0815939607448\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
117	-67.0815939607448\\
118	-67.2217968943284\\
119	-67.3797975189083\\
120	-67.5284341462029\\
121	-67.3815936066283\\
122	-68.0763628489194\\
123	-68.3761739012275\\
124	-69.0203398802649\\
125	-69.2809200814939\\
126	-69.1870607467771\\
127	-69.775349780907\\
128	-70.1796999577279\\
129	-69.246345334302\\
130	-70.0202276287842\\
131	-69.9819084264758\\
132	-69.0368687149802\\
133	-69.4236170625675\\
134	-69.8103654101549\\
135	-70.3922801998731\\
136	-71.1038053443635\\
137	-70.5481572189764\\
138	-70.6880479298702\\
139	-70.3398807275227\\
140	-70.9663424241973\\
141	-71.1144026229873\\
142	-70.9228209633137\\
143	-70.9018359319728\\
144	-70.4347189913394\\
145	-69.5859644438928\\
146	-69.6732629139434\\
147	-69.9476153752139\\
148	-69.7386116183021\\
149	-69.4159510962011\\
150	-70.3102536929679\\
151	-70.1399360447471\\
152	-70.5306987914261\\
153	-70.5577615700592\\
154	-70.4632155545321\\
155	-70.1878617528379\\
156	-69.9731754009764\\
157	-69.3499959377805\\
158	-68.6149799837247\\
159	-68.2499410764949\\
160	-68.7788976728229\\
161	-69.9201202255042\\
162	-69.949384556793\\
163	-69.6084014012527\\
164	-69.2131758822892\\
165	-69.259167712789\\
166	-68.5902285123349\\
167	-68.761934276738\\
168	-68.269149385256\\
169	-67.2641216314658\\
170	-66.6611335026917\\
171	-67.5860114696867\\
172	-67.8180865441316\\
173	-67.0864136629009\\
174	-67.0640523632081\\
175	-66.8225013104416\\
176	-66.8272218572073\\
177	-66.5241824179815\\
178	-66.2488463147484\\
179	-66.4433050563089\\
180	-67.5088289875535\\
181	-67.4438487435193\\
182	-67.7461492977076\\
183	-67.3264709383901\\
184	-67.4054949091177\\
185	-66.9752099100331\\
186	-66.3621143907475\\
187	-66.2562474609941\\
188	-67.1438956118309\\
189	-67.0922906661262\\
189	-67.0922906661262\\
189	-72\\
117	-72\\
117	-67.0815939607448\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
120	-67.5284341462029\\
121	-67.3815936066283\\
122	-68.0763628489194\\
123	-68.3761739012275\\
124	-69.0203398802649\\
125	-69.2809200814939\\
126	-69.1870607467771\\
127	-69.775349780907\\
128	-70.1796999577279\\
129	-69.246345334302\\
130	-70.0202276287842\\
131	-69.9819084264758\\
132	-69.0368687149802\\
133	-69.4236170625675\\
134	-69.8103654101549\\
135	-70.3922801998731\\
136	-71.1038053443635\\
137	-70.5481572189764\\
138	-70.6880479298702\\
139	-70.3398807275227\\
140	-70.9663424241973\\
141	-71.1144026229873\\
142	-70.9228209633137\\
143	-70.9018359319728\\
144	-70.4347189913394\\
145	-69.5859644438928\\
146	-69.6732629139434\\
147	-69.9476153752139\\
148	-69.7386116183021\\
149	-69.4159510962011\\
150	-70.3102536929679\\
151	-70.1399360447471\\
152	-70.5306987914261\\
153	-70.5577615700592\\
154	-70.4632155545321\\
155	-70.1878617528379\\
156	-69.9731754009764\\
157	-69.3499959377805\\
158	-68.6149799837247\\
159	-68.2499410764949\\
160	-68.7788976728229\\
161	-69.9201202255042\\
162	-69.949384556793\\
163	-69.6084014012527\\
164	-69.2131758822892\\
165	-69.259167712789\\
166	-68.5902285123349\\
167	-68.761934276738\\
168	-68.269149385256\\
169	-67.2641216314658\\
170	-66.6611335026917\\
171	-67.5860114696867\\
172	-67.8180865441316\\
173	-67.0864136629009\\
174	-67.0640523632081\\
175	-66.8225013104416\\
176	-66.8272218572073\\
177	-66.5241824179815\\
178	-66.2488463147484\\
179	-66.4433050563089\\
180	-67.5088289875535\\
181	-67.4438487435193\\
182	-67.7461492977076\\
183	-67.3264709383901\\
184	-67.4054949091177\\
185	-66.9752099100331\\
186	-66.3621143907475\\
187	-66.2562474609941\\
188	-67.1438956118309\\
189	-67.0922906661262\\
189	-67.0922906661262\\
189	-72\\
120	-72\\
120	-67.5284341462029\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
120	-67.5284341462029\\
121	-67.3815936066283\\
122	-68.0763628489194\\
123	-68.3761739012275\\
124	-69.0203398802649\\
125	-69.2809200814939\\
126	-69.1870607467771\\
127	-69.775349780907\\
128	-70.1796999577279\\
129	-69.246345334302\\
130	-70.0202276287842\\
131	-69.9819084264758\\
132	-69.0368687149802\\
133	-69.4236170625675\\
134	-69.8103654101549\\
135	-70.3922801998731\\
136	-71.1038053443635\\
137	-70.5481572189764\\
138	-70.6880479298702\\
139	-70.3398807275227\\
140	-70.9663424241973\\
141	-71.1144026229873\\
142	-70.9228209633137\\
143	-70.9018359319728\\
144	-70.4347189913394\\
145	-69.5859644438928\\
146	-69.6732629139434\\
147	-69.9476153752139\\
148	-69.7386116183021\\
149	-69.4159510962011\\
150	-70.3102536929679\\
151	-70.1399360447471\\
152	-70.5306987914261\\
153	-70.5577615700592\\
154	-70.4632155545321\\
155	-70.1878617528379\\
156	-69.9731754009764\\
157	-69.3499959377805\\
158	-68.6149799837247\\
159	-68.2499410764949\\
160	-68.7788976728229\\
161	-69.9201202255042\\
162	-69.949384556793\\
163	-69.6084014012527\\
164	-69.2131758822892\\
165	-69.259167712789\\
166	-68.5902285123349\\
167	-68.761934276738\\
168	-68.269149385256\\
169	-67.2641216314658\\
170	-66.6611335026917\\
171	-67.5860114696867\\
172	-67.8180865441316\\
173	-67.0864136629009\\
174	-67.0640523632081\\
175	-66.8225013104416\\
176	-66.8272218572073\\
177	-66.5241824179815\\
178	-66.2488463147484\\
179	-66.4433050563089\\
180	-67.5088289875535\\
181	-67.4438487435193\\
182	-67.7461492977076\\
183	-67.3264709383901\\
184	-67.4054949091177\\
185	-66.9752099100331\\
186	-66.3621143907475\\
187	-66.2562474609941\\
188	-67.1438956118309\\
189	-67.0922906661262\\
189	-67.0922906661262\\
189	-72\\
120	-72\\
120	-67.5284341462029\\
}--cycle;

\addplot[area legend, draw=none, fill=black, fill opacity=\shadowOpacity, forget plot]
table[row sep=crcr] {%
x	y\\
120	-67.5284341462029\\
121	-67.3815936066283\\
122	-68.0763628489194\\
123	-68.3761739012275\\
124	-69.0203398802649\\
125	-69.2809200814939\\
126	-69.1870607467771\\
127	-69.775349780907\\
128	-70.1796999577279\\
129	-69.246345334302\\
130	-70.0202276287842\\
131	-69.9819084264758\\
132	-69.0368687149802\\
133	-69.4236170625675\\
134	-69.8103654101549\\
135	-70.3922801998731\\
136	-71.1038053443635\\
137	-70.5481572189764\\
138	-70.6880479298702\\
139	-70.3398807275227\\
140	-70.9663424241973\\
141	-71.1144026229873\\
142	-70.9228209633137\\
143	-70.9018359319728\\
144	-70.4347189913394\\
145	-69.5859644438928\\
146	-69.6732629139434\\
147	-69.9476153752139\\
148	-69.7386116183021\\
149	-69.4159510962011\\
150	-70.3102536929679\\
151	-70.1399360447471\\
152	-70.5306987914261\\
153	-70.5577615700592\\
154	-70.4632155545321\\
155	-70.1878617528379\\
156	-69.9731754009764\\
157	-69.3499959377805\\
158	-68.6149799837247\\
159	-68.2499410764949\\
160	-68.7788976728229\\
161	-69.9201202255042\\
162	-69.949384556793\\
163	-69.6084014012527\\
164	-69.2131758822892\\
165	-69.259167712789\\
166	-68.5902285123349\\
167	-68.761934276738\\
168	-68.269149385256\\
169	-67.2641216314658\\
170	-66.6611335026917\\
171	-67.5860114696867\\
172	-67.8180865441316\\
173	-67.0864136629009\\
174	-67.0640523632081\\
175	-66.8225013104416\\
176	-66.8272218572073\\
177	-66.5241824179815\\
178	-66.2488463147484\\
179	-66.4433050563089\\
180	-67.5088289875535\\
181	-67.4438487435193\\
182	-67.7461492977076\\
183	-67.3264709383901\\
184	-67.4054949091177\\
185	-66.9752099100331\\
186	-66.3621143907475\\
187	-66.2562474609941\\
188	-67.1438956118309\\
189	-67.0922906661262\\
189	-67.0922906661262\\
189	-72\\
120	-72\\
120	-67.5284341462029\\
}--cycle;


==> figures/subarrays-only.tex <==


\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4472714285714	-1.63975	3.09908333333333\\
15.4472714285714	-1.86225	3.09908333333333\\
15.4472714285714	-1.86225	3.32158333333333\\
15.4472714285714	-1.63975	3.32158333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-1.63975	3.09908333333333\\
15.4727	-1.86225	3.09908333333333\\
15.4727	-1.86225	3.32158333333333\\
15.4727	-1.63975	3.32158333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-1.63975	3.09908333333333\\
15.4727	-1.86225	3.09908333333333\\
15.4472714285714	-1.86225	3.09908333333333\\
15.4472714285714	-1.63975	3.09908333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-1.63975	3.32158333333333\\
15.4727	-1.86225	3.32158333333333\\
15.4472714285714	-1.86225	3.32158333333333\\
15.4472714285714	-1.63975	3.32158333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-1.63975	3.09908333333333\\
15.4727	-1.63975	3.32158333333333\\
15.4472714285714	-1.63975	3.32158333333333\\
15.4472714285714	-1.63975	3.09908333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-1.86225	3.09908333333333\\
15.4727	-1.86225	3.32158333333333\\
15.4472714285714	-1.86225	3.32158333333333\\
15.4472714285714	-1.86225	3.09908333333333\\
}--cycle;
\addplot3 [color=subarrayorange, only marks, mark=*, mark size = 0.1pt, mark options={solid}, line width = 0pt, mark options={solid, subarrayorange}]
 table[row sep=crcr] {%
15.446	-1.6635	3.29783333333333\\
15.446	-1.6885	3.29783333333333\\
15.446	-1.7135	3.29783333333333\\
15.446	-1.7385	3.29783333333333\\
15.446	-1.7635	3.29783333333333\\
15.446	-1.7885	3.29783333333333\\
15.446	-1.8135	3.29783333333333\\
15.446	-1.8385	3.29783333333333\\
15.446	-1.6635	3.27283333333333\\
15.446	-1.6885	3.27283333333333\\
15.446	-1.7135	3.27283333333333\\
15.446	-1.7385	3.27283333333333\\
15.446	-1.7635	3.27283333333333\\
15.446	-1.7885	3.27283333333333\\
15.446	-1.8135	3.27283333333333\\
15.446	-1.8385	3.27283333333333\\
15.446	-1.6635	3.24783333333333\\
15.446	-1.6885	3.24783333333333\\
15.446	-1.7135	3.24783333333333\\
15.446	-1.7385	3.24783333333333\\
15.446	-1.7635	3.24783333333333\\
15.446	-1.7885	3.24783333333333\\
15.446	-1.8135	3.24783333333333\\
15.446	-1.8385	3.24783333333333\\
15.446	-1.6635	3.22283333333333\\
15.446	-1.6885	3.22283333333333\\
15.446	-1.7135	3.22283333333333\\
15.446	-1.7385	3.22283333333333\\
15.446	-1.7635	3.22283333333333\\
15.446	-1.7885	3.22283333333333\\
15.446	-1.8135	3.22283333333333\\
15.446	-1.8385	3.22283333333333\\
15.446	-1.6635	3.19783333333333\\
15.446	-1.6885	3.19783333333333\\
15.446	-1.7135	3.19783333333333\\
15.446	-1.7385	3.19783333333333\\
15.446	-1.7635	3.19783333333333\\
15.446	-1.7885	3.19783333333333\\
15.446	-1.8135	3.19783333333333\\
15.446	-1.8385	3.19783333333333\\
15.446	-1.6635	3.17283333333333\\
15.446	-1.6885	3.17283333333333\\
15.446	-1.7135	3.17283333333333\\
15.446	-1.7385	3.17283333333333\\
15.446	-1.7635	3.17283333333333\\
15.446	-1.7885	3.17283333333333\\
15.446	-1.8135	3.17283333333333\\
15.446	-1.8385	3.17283333333333\\
15.446	-1.6635	3.14783333333333\\
15.446	-1.6885	3.14783333333333\\
15.446	-1.7135	3.14783333333333\\
15.446	-1.7385	3.14783333333333\\
15.446	-1.7635	3.14783333333333\\
15.446	-1.7885	3.14783333333333\\
15.446	-1.8135	3.14783333333333\\
15.446	-1.8385	3.14783333333333\\
15.446	-1.6635	3.12283333333333\\
15.446	-1.6885	3.12283333333333\\
15.446	-1.7135	3.12283333333333\\
15.446	-1.7385	3.12283333333333\\
15.446	-1.7635	3.12283333333333\\
15.446	-1.7885	3.12283333333333\\
15.446	-1.8135	3.12283333333333\\
15.446	-1.8385	3.12283333333333\\
};
 
\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4472714285714	-1.63975	3.61575\\
15.4472714285714	-1.86225	3.61575\\
15.4472714285714	-1.86225	3.83825\\
15.4472714285714	-1.63975	3.83825\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-1.63975	3.61575\\
15.4727	-1.86225	3.61575\\
15.4727	-1.86225	3.83825\\
15.4727	-1.63975	3.83825\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-1.63975	3.61575\\
15.4727	-1.86225	3.61575\\
15.4472714285714	-1.86225	3.61575\\
15.4472714285714	-1.63975	3.61575\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-1.63975	3.83825\\
15.4727	-1.86225	3.83825\\
15.4472714285714	-1.86225	3.83825\\
15.4472714285714	-1.63975	3.83825\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-1.63975	3.61575\\
15.4727	-1.63975	3.83825\\
15.4472714285714	-1.63975	3.83825\\
15.4472714285714	-1.63975	3.61575\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-1.86225	3.61575\\
15.4727	-1.86225	3.83825\\
15.4472714285714	-1.86225	3.83825\\
15.4472714285714	-1.86225	3.61575\\
}--cycle;
\addplot3 [color=subarrayorange, only marks, mark=*, mark size = 0.1pt, mark options={solid}, line width = 0pt, mark options={solid, subarrayorange}]
 table[row sep=crcr] {%
15.446	-1.6635	3.8145\\
15.446	-1.6885	3.8145\\
15.446	-1.7135	3.8145\\
15.446	-1.7385	3.8145\\
15.446	-1.7635	3.8145\\
15.446	-1.7885	3.8145\\
15.446	-1.8135	3.8145\\
15.446	-1.8385	3.8145\\
15.446	-1.6635	3.7895\\
15.446	-1.6885	3.7895\\
15.446	-1.7135	3.7895\\
15.446	-1.7385	3.7895\\
15.446	-1.7635	3.7895\\
15.446	-1.7885	3.7895\\
15.446	-1.8135	3.7895\\
15.446	-1.8385	3.7895\\
15.446	-1.6635	3.7645\\
15.446	-1.6885	3.7645\\
15.446	-1.7135	3.7645\\
15.446	-1.7385	3.7645\\
15.446	-1.7635	3.7645\\
15.446	-1.7885	3.7645\\
15.446	-1.8135	3.7645\\
15.446	-1.8385	3.7645\\
15.446	-1.6635	3.7395\\
15.446	-1.6885	3.7395\\
15.446	-1.7135	3.7395\\
15.446	-1.7385	3.7395\\
15.446	-1.7635	3.7395\\
15.446	-1.7885	3.7395\\
15.446	-1.8135	3.7395\\
15.446	-1.8385	3.7395\\
15.446	-1.6635	3.7145\\
15.446	-1.6885	3.7145\\
15.446	-1.7135	3.7145\\
15.446	-1.7385	3.7145\\
15.446	-1.7635	3.7145\\
15.446	-1.7885	3.7145\\
15.446	-1.8135	3.7145\\
15.446	-1.8385	3.7145\\
15.446	-1.6635	3.6895\\
15.446	-1.6885	3.6895\\
15.446	-1.7135	3.6895\\
15.446	-1.7385	3.6895\\
15.446	-1.7635	3.6895\\
15.446	-1.7885	3.6895\\
15.446	-1.8135	3.6895\\
15.446	-1.8385	3.6895\\
15.446	-1.6635	3.6645\\
15.446	-1.6885	3.6645\\
15.446	-1.7135	3.6645\\
15.446	-1.7385	3.6645\\
15.446	-1.7635	3.6645\\
15.446	-1.7885	3.6645\\
15.446	-1.8135	3.6645\\
15.446	-1.8385	3.6645\\
15.446	-1.6635	3.6395\\
15.446	-1.6885	3.6395\\
15.446	-1.7135	3.6395\\
15.446	-1.7385	3.6395\\
15.446	-1.7635	3.6395\\
15.446	-1.7885	3.6395\\
15.446	-1.8135	3.6395\\
15.446	-1.8385	3.6395\\
};
 
\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4472714285714	-1.63975	4.13241666666667\\
15.4472714285714	-1.86225	4.13241666666667\\
15.4472714285714	-1.86225	4.35491666666667\\
15.4472714285714	-1.63975	4.35491666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-1.63975	4.13241666666667\\
15.4727	-1.86225	4.13241666666667\\
15.4727	-1.86225	4.35491666666667\\
15.4727	-1.63975	4.35491666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-1.63975	4.13241666666667\\
15.4727	-1.86225	4.13241666666667\\
15.4472714285714	-1.86225	4.13241666666667\\
15.4472714285714	-1.63975	4.13241666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-1.63975	4.35491666666667\\
15.4727	-1.86225	4.35491666666667\\
15.4472714285714	-1.86225	4.35491666666667\\
15.4472714285714	-1.63975	4.35491666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-1.63975	4.13241666666667\\
15.4727	-1.63975	4.35491666666667\\
15.4472714285714	-1.63975	4.35491666666667\\
15.4472714285714	-1.63975	4.13241666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-1.86225	4.13241666666667\\
15.4727	-1.86225	4.35491666666667\\
15.4472714285714	-1.86225	4.35491666666667\\
15.4472714285714	-1.86225	4.13241666666667\\
}--cycle;
\addplot3 [color=subarrayorange, only marks, mark=*, mark size = 0.1pt, mark options={solid}, line width = 0pt, mark options={solid, subarrayorange}]
 table[row sep=crcr] {%
15.446	-1.6635	4.33116666666667\\
15.446	-1.6885	4.33116666666667\\
15.446	-1.7135	4.33116666666667\\
15.446	-1.7385	4.33116666666667\\
15.446	-1.7635	4.33116666666667\\
15.446	-1.7885	4.33116666666667\\
15.446	-1.8135	4.33116666666667\\
15.446	-1.8385	4.33116666666667\\
15.446	-1.6635	4.30616666666667\\
15.446	-1.6885	4.30616666666667\\
15.446	-1.7135	4.30616666666667\\
15.446	-1.7385	4.30616666666667\\
15.446	-1.7635	4.30616666666667\\
15.446	-1.7885	4.30616666666667\\
15.446	-1.8135	4.30616666666667\\
15.446	-1.8385	4.30616666666667\\
15.446	-1.6635	4.28116666666667\\
15.446	-1.6885	4.28116666666667\\
15.446	-1.7135	4.28116666666667\\
15.446	-1.7385	4.28116666666667\\
15.446	-1.7635	4.28116666666667\\
15.446	-1.7885	4.28116666666667\\
15.446	-1.8135	4.28116666666667\\
15.446	-1.8385	4.28116666666667\\
15.446	-1.6635	4.25616666666667\\
15.446	-1.6885	4.25616666666667\\
15.446	-1.7135	4.25616666666667\\
15.446	-1.7385	4.25616666666667\\
15.446	-1.7635	4.25616666666667\\
15.446	-1.7885	4.25616666666667\\
15.446	-1.8135	4.25616666666667\\
15.446	-1.8385	4.25616666666667\\
15.446	-1.6635	4.23116666666667\\
15.446	-1.6885	4.23116666666667\\
15.446	-1.7135	4.23116666666667\\
15.446	-1.7385	4.23116666666667\\
15.446	-1.7635	4.23116666666667\\
15.446	-1.7885	4.23116666666667\\
15.446	-1.8135	4.23116666666667\\
15.446	-1.8385	4.23116666666667\\
15.446	-1.6635	4.20616666666667\\
15.446	-1.6885	4.20616666666667\\
15.446	-1.7135	4.20616666666667\\
15.446	-1.7385	4.20616666666667\\
15.446	-1.7635	4.20616666666667\\
15.446	-1.7885	4.20616666666667\\
15.446	-1.8135	4.20616666666667\\
15.446	-1.8385	4.20616666666667\\
15.446	-1.6635	4.18116666666667\\
15.446	-1.6885	4.18116666666667\\
15.446	-1.7135	4.18116666666667\\
15.446	-1.7385	4.18116666666667\\
15.446	-1.7635	4.18116666666667\\
15.446	-1.7885	4.18116666666667\\
15.446	-1.8135	4.18116666666667\\
15.446	-1.8385	4.18116666666667\\
15.446	-1.6635	4.15616666666667\\
15.446	-1.6885	4.15616666666667\\
15.446	-1.7135	4.15616666666667\\
15.446	-1.7385	4.15616666666667\\
15.446	-1.7635	4.15616666666667\\
15.446	-1.7885	4.15616666666667\\
15.446	-1.8135	4.15616666666667\\
15.446	-1.8385	4.15616666666667\\
};
 
\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4472714285714	-2.09175	3.09908333333333\\
15.4472714285714	-2.31425	3.09908333333333\\
15.4472714285714	-2.31425	3.32158333333333\\
15.4472714285714	-2.09175	3.32158333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.09175	3.09908333333333\\
15.4727	-2.31425	3.09908333333333\\
15.4727	-2.31425	3.32158333333333\\
15.4727	-2.09175	3.32158333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.09175	3.09908333333333\\
15.4727	-2.31425	3.09908333333333\\
15.4472714285714	-2.31425	3.09908333333333\\
15.4472714285714	-2.09175	3.09908333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.09175	3.32158333333333\\
15.4727	-2.31425	3.32158333333333\\
15.4472714285714	-2.31425	3.32158333333333\\
15.4472714285714	-2.09175	3.32158333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.09175	3.09908333333333\\
15.4727	-2.09175	3.32158333333333\\
15.4472714285714	-2.09175	3.32158333333333\\
15.4472714285714	-2.09175	3.09908333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.31425	3.09908333333333\\
15.4727	-2.31425	3.32158333333333\\
15.4472714285714	-2.31425	3.32158333333333\\
15.4472714285714	-2.31425	3.09908333333333\\
}--cycle;
\addplot3 [color=subarrayorange, only marks, mark=*, mark size = 0.1pt, mark options={solid}, line width = 0pt, mark options={solid, subarrayorange}]
 table[row sep=crcr] {%
15.446	-2.1155	3.29783333333333\\
15.446	-2.1405	3.29783333333333\\
15.446	-2.1655	3.29783333333333\\
15.446	-2.1905	3.29783333333333\\
15.446	-2.2155	3.29783333333333\\
15.446	-2.2405	3.29783333333333\\
15.446	-2.2655	3.29783333333333\\
15.446	-2.2905	3.29783333333333\\
15.446	-2.1155	3.27283333333333\\
15.446	-2.1405	3.27283333333333\\
15.446	-2.1655	3.27283333333333\\
15.446	-2.1905	3.27283333333333\\
15.446	-2.2155	3.27283333333333\\
15.446	-2.2405	3.27283333333333\\
15.446	-2.2655	3.27283333333333\\
15.446	-2.2905	3.27283333333333\\
15.446	-2.1155	3.24783333333333\\
15.446	-2.1405	3.24783333333333\\
15.446	-2.1655	3.24783333333333\\
15.446	-2.1905	3.24783333333333\\
15.446	-2.2155	3.24783333333333\\
15.446	-2.2405	3.24783333333333\\
15.446	-2.2655	3.24783333333333\\
15.446	-2.2905	3.24783333333333\\
15.446	-2.1155	3.22283333333333\\
15.446	-2.1405	3.22283333333333\\
15.446	-2.1655	3.22283333333333\\
15.446	-2.1905	3.22283333333333\\
15.446	-2.2155	3.22283333333333\\
15.446	-2.2405	3.22283333333333\\
15.446	-2.2655	3.22283333333333\\
15.446	-2.2905	3.22283333333333\\
15.446	-2.1155	3.19783333333333\\
15.446	-2.1405	3.19783333333333\\
15.446	-2.1655	3.19783333333333\\
15.446	-2.1905	3.19783333333333\\
15.446	-2.2155	3.19783333333333\\
15.446	-2.2405	3.19783333333333\\
15.446	-2.2655	3.19783333333333\\
15.446	-2.2905	3.19783333333333\\
15.446	-2.1155	3.17283333333333\\
15.446	-2.1405	3.17283333333333\\
15.446	-2.1655	3.17283333333333\\
15.446	-2.1905	3.17283333333333\\
15.446	-2.2155	3.17283333333333\\
15.446	-2.2405	3.17283333333333\\
15.446	-2.2655	3.17283333333333\\
15.446	-2.2905	3.17283333333333\\
15.446	-2.1155	3.14783333333333\\
15.446	-2.1405	3.14783333333333\\
15.446	-2.1655	3.14783333333333\\
15.446	-2.1905	3.14783333333333\\
15.446	-2.2155	3.14783333333333\\
15.446	-2.2405	3.14783333333333\\
15.446	-2.2655	3.14783333333333\\
15.446	-2.2905	3.14783333333333\\
15.446	-2.1155	3.12283333333333\\
15.446	-2.1405	3.12283333333333\\
15.446	-2.1655	3.12283333333333\\
15.446	-2.1905	3.12283333333333\\
15.446	-2.2155	3.12283333333333\\
15.446	-2.2405	3.12283333333333\\
15.446	-2.2655	3.12283333333333\\
15.446	-2.2905	3.12283333333333\\
};
 
\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4472714285714	-2.09175	3.61575\\
15.4472714285714	-2.31425	3.61575\\
15.4472714285714	-2.31425	3.83825\\
15.4472714285714	-2.09175	3.83825\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.09175	3.61575\\
15.4727	-2.31425	3.61575\\
15.4727	-2.31425	3.83825\\
15.4727	-2.09175	3.83825\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.09175	3.61575\\
15.4727	-2.31425	3.61575\\
15.4472714285714	-2.31425	3.61575\\
15.4472714285714	-2.09175	3.61575\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.09175	3.83825\\
15.4727	-2.31425	3.83825\\
15.4472714285714	-2.31425	3.83825\\
15.4472714285714	-2.09175	3.83825\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.09175	3.61575\\
15.4727	-2.09175	3.83825\\
15.4472714285714	-2.09175	3.83825\\
15.4472714285714	-2.09175	3.61575\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.31425	3.61575\\
15.4727	-2.31425	3.83825\\
15.4472714285714	-2.31425	3.83825\\
15.4472714285714	-2.31425	3.61575\\
}--cycle;
\addplot3 [color=subarrayorange, only marks, mark=*, mark size = 0.1pt, mark options={solid}, line width = 0pt, mark options={solid, subarrayorange}]
 table[row sep=crcr] {%
15.446	-2.1155	3.8145\\
15.446	-2.1405	3.8145\\
15.446	-2.1655	3.8145\\
15.446	-2.1905	3.8145\\
15.446	-2.2155	3.8145\\
15.446	-2.2405	3.8145\\
15.446	-2.2655	3.8145\\
15.446	-2.2905	3.8145\\
15.446	-2.1155	3.7895\\
15.446	-2.1405	3.7895\\
15.446	-2.1655	3.7895\\
15.446	-2.1905	3.7895\\
15.446	-2.2155	3.7895\\
15.446	-2.2405	3.7895\\
15.446	-2.2655	3.7895\\
15.446	-2.2905	3.7895\\
15.446	-2.1155	3.7645\\
15.446	-2.1405	3.7645\\
15.446	-2.1655	3.7645\\
15.446	-2.1905	3.7645\\
15.446	-2.2155	3.7645\\
15.446	-2.2405	3.7645\\
15.446	-2.2655	3.7645\\
15.446	-2.2905	3.7645\\
15.446	-2.1155	3.7395\\
15.446	-2.1405	3.7395\\
15.446	-2.1655	3.7395\\
15.446	-2.1905	3.7395\\
15.446	-2.2155	3.7395\\
15.446	-2.2405	3.7395\\
15.446	-2.2655	3.7395\\
15.446	-2.2905	3.7395\\
15.446	-2.1155	3.7145\\
15.446	-2.1405	3.7145\\
15.446	-2.1655	3.7145\\
15.446	-2.1905	3.7145\\
15.446	-2.2155	3.7145\\
15.446	-2.2405	3.7145\\
15.446	-2.2655	3.7145\\
15.446	-2.2905	3.7145\\
15.446	-2.1155	3.6895\\
15.446	-2.1405	3.6895\\
15.446	-2.1655	3.6895\\
15.446	-2.1905	3.6895\\
15.446	-2.2155	3.6895\\
15.446	-2.2405	3.6895\\
15.446	-2.2655	3.6895\\
15.446	-2.2905	3.6895\\
15.446	-2.1155	3.6645\\
15.446	-2.1405	3.6645\\
15.446	-2.1655	3.6645\\
15.446	-2.1905	3.6645\\
15.446	-2.2155	3.6645\\
15.446	-2.2405	3.6645\\
15.446	-2.2655	3.6645\\
15.446	-2.2905	3.6645\\
15.446	-2.1155	3.6395\\
15.446	-2.1405	3.6395\\
15.446	-2.1655	3.6395\\
15.446	-2.1905	3.6395\\
15.446	-2.2155	3.6395\\
15.446	-2.2405	3.6395\\
15.446	-2.2655	3.6395\\
15.446	-2.2905	3.6395\\
};
 
\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4472714285714	-2.09175	4.13241666666667\\
15.4472714285714	-2.31425	4.13241666666667\\
15.4472714285714	-2.31425	4.35491666666667\\
15.4472714285714	-2.09175	4.35491666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.09175	4.13241666666667\\
15.4727	-2.31425	4.13241666666667\\
15.4727	-2.31425	4.35491666666667\\
15.4727	-2.09175	4.35491666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.09175	4.13241666666667\\
15.4727	-2.31425	4.13241666666667\\
15.4472714285714	-2.31425	4.13241666666667\\
15.4472714285714	-2.09175	4.13241666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.09175	4.35491666666667\\
15.4727	-2.31425	4.35491666666667\\
15.4472714285714	-2.31425	4.35491666666667\\
15.4472714285714	-2.09175	4.35491666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.09175	4.13241666666667\\
15.4727	-2.09175	4.35491666666667\\
15.4472714285714	-2.09175	4.35491666666667\\
15.4472714285714	-2.09175	4.13241666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.31425	4.13241666666667\\
15.4727	-2.31425	4.35491666666667\\
15.4472714285714	-2.31425	4.35491666666667\\
15.4472714285714	-2.31425	4.13241666666667\\
}--cycle;
\addplot3 [color=subarrayorange, only marks, mark=*, mark size = 0.1pt, mark options={solid}, line width = 0pt, mark options={solid, subarrayorange}]
 table[row sep=crcr] {%
15.446	-2.1155	4.33116666666667\\
15.446	-2.1405	4.33116666666667\\
15.446	-2.1655	4.33116666666667\\
15.446	-2.1905	4.33116666666667\\
15.446	-2.2155	4.33116666666667\\
15.446	-2.2405	4.33116666666667\\
15.446	-2.2655	4.33116666666667\\
15.446	-2.2905	4.33116666666667\\
15.446	-2.1155	4.30616666666667\\
15.446	-2.1405	4.30616666666667\\
15.446	-2.1655	4.30616666666667\\
15.446	-2.1905	4.30616666666667\\
15.446	-2.2155	4.30616666666667\\
15.446	-2.2405	4.30616666666667\\
15.446	-2.2655	4.30616666666667\\
15.446	-2.2905	4.30616666666667\\
15.446	-2.1155	4.28116666666667\\
15.446	-2.1405	4.28116666666667\\
15.446	-2.1655	4.28116666666667\\
15.446	-2.1905	4.28116666666667\\
15.446	-2.2155	4.28116666666667\\
15.446	-2.2405	4.28116666666667\\
15.446	-2.2655	4.28116666666667\\
15.446	-2.2905	4.28116666666667\\
15.446	-2.1155	4.25616666666667\\
15.446	-2.1405	4.25616666666667\\
15.446	-2.1655	4.25616666666667\\
15.446	-2.1905	4.25616666666667\\
15.446	-2.2155	4.25616666666667\\
15.446	-2.2405	4.25616666666667\\
15.446	-2.2655	4.25616666666667\\
15.446	-2.2905	4.25616666666667\\
15.446	-2.1155	4.23116666666667\\
15.446	-2.1405	4.23116666666667\\
15.446	-2.1655	4.23116666666667\\
15.446	-2.1905	4.23116666666667\\
15.446	-2.2155	4.23116666666667\\
15.446	-2.2405	4.23116666666667\\
15.446	-2.2655	4.23116666666667\\
15.446	-2.2905	4.23116666666667\\
15.446	-2.1155	4.20616666666667\\
15.446	-2.1405	4.20616666666667\\
15.446	-2.1655	4.20616666666667\\
15.446	-2.1905	4.20616666666667\\
15.446	-2.2155	4.20616666666667\\
15.446	-2.2405	4.20616666666667\\
15.446	-2.2655	4.20616666666667\\
15.446	-2.2905	4.20616666666667\\
15.446	-2.1155	4.18116666666667\\
15.446	-2.1405	4.18116666666667\\
15.446	-2.1655	4.18116666666667\\
15.446	-2.1905	4.18116666666667\\
15.446	-2.2155	4.18116666666667\\
15.446	-2.2405	4.18116666666667\\
15.446	-2.2655	4.18116666666667\\
15.446	-2.2905	4.18116666666667\\
15.446	-2.1155	4.15616666666667\\
15.446	-2.1405	4.15616666666667\\
15.446	-2.1655	4.15616666666667\\
15.446	-2.1905	4.15616666666667\\
15.446	-2.2155	4.15616666666667\\
15.446	-2.2405	4.15616666666667\\
15.446	-2.2655	4.15616666666667\\
15.446	-2.2905	4.15616666666667\\
};
 
\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4472714285714	-2.54375	3.09908333333333\\
15.4472714285714	-2.76625	3.09908333333333\\
15.4472714285714	-2.76625	3.32158333333333\\
15.4472714285714	-2.54375	3.32158333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.54375	3.09908333333333\\
15.4727	-2.76625	3.09908333333333\\
15.4727	-2.76625	3.32158333333333\\
15.4727	-2.54375	3.32158333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.54375	3.09908333333333\\
15.4727	-2.76625	3.09908333333333\\
15.4472714285714	-2.76625	3.09908333333333\\
15.4472714285714	-2.54375	3.09908333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.54375	3.32158333333333\\
15.4727	-2.76625	3.32158333333333\\
15.4472714285714	-2.76625	3.32158333333333\\
15.4472714285714	-2.54375	3.32158333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.54375	3.09908333333333\\
15.4727	-2.54375	3.32158333333333\\
15.4472714285714	-2.54375	3.32158333333333\\
15.4472714285714	-2.54375	3.09908333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.76625	3.09908333333333\\
15.4727	-2.76625	3.32158333333333\\
15.4472714285714	-2.76625	3.32158333333333\\
15.4472714285714	-2.76625	3.09908333333333\\
}--cycle;
\addplot3 [color=subarrayorange, only marks, mark=*, mark size = 0.1pt, mark options={solid}, line width = 0pt, mark options={solid, subarrayorange}]
 table[row sep=crcr] {%
15.446	-2.5675	3.29783333333333\\
15.446	-2.5925	3.29783333333333\\
15.446	-2.6175	3.29783333333333\\
15.446	-2.6425	3.29783333333333\\
15.446	-2.6675	3.29783333333333\\
15.446	-2.6925	3.29783333333333\\
15.446	-2.7175	3.29783333333333\\
15.446	-2.7425	3.29783333333333\\
15.446	-2.5675	3.27283333333333\\
15.446	-2.5925	3.27283333333333\\
15.446	-2.6175	3.27283333333333\\
15.446	-2.6425	3.27283333333333\\
15.446	-2.6675	3.27283333333333\\
15.446	-2.6925	3.27283333333333\\
15.446	-2.7175	3.27283333333333\\
15.446	-2.7425	3.27283333333333\\
15.446	-2.5675	3.24783333333333\\
15.446	-2.5925	3.24783333333333\\
15.446	-2.6175	3.24783333333333\\
15.446	-2.6425	3.24783333333333\\
15.446	-2.6675	3.24783333333333\\
15.446	-2.6925	3.24783333333333\\
15.446	-2.7175	3.24783333333333\\
15.446	-2.7425	3.24783333333333\\
15.446	-2.5675	3.22283333333333\\
15.446	-2.5925	3.22283333333333\\
15.446	-2.6175	3.22283333333333\\
15.446	-2.6425	3.22283333333333\\
15.446	-2.6675	3.22283333333333\\
15.446	-2.6925	3.22283333333333\\
15.446	-2.7175	3.22283333333333\\
15.446	-2.7425	3.22283333333333\\
15.446	-2.5675	3.19783333333333\\
15.446	-2.5925	3.19783333333333\\
15.446	-2.6175	3.19783333333333\\
15.446	-2.6425	3.19783333333333\\
15.446	-2.6675	3.19783333333333\\
15.446	-2.6925	3.19783333333333\\
15.446	-2.7175	3.19783333333333\\
15.446	-2.7425	3.19783333333333\\
15.446	-2.5675	3.17283333333333\\
15.446	-2.5925	3.17283333333333\\
15.446	-2.6175	3.17283333333333\\
15.446	-2.6425	3.17283333333333\\
15.446	-2.6675	3.17283333333333\\
15.446	-2.6925	3.17283333333333\\
15.446	-2.7175	3.17283333333333\\
15.446	-2.7425	3.17283333333333\\
15.446	-2.5675	3.14783333333333\\
15.446	-2.5925	3.14783333333333\\
15.446	-2.6175	3.14783333333333\\
15.446	-2.6425	3.14783333333333\\
15.446	-2.6675	3.14783333333333\\
15.446	-2.6925	3.14783333333333\\
15.446	-2.7175	3.14783333333333\\
15.446	-2.7425	3.14783333333333\\
15.446	-2.5675	3.12283333333333\\
15.446	-2.5925	3.12283333333333\\
15.446	-2.6175	3.12283333333333\\
15.446	-2.6425	3.12283333333333\\
15.446	-2.6675	3.12283333333333\\
15.446	-2.6925	3.12283333333333\\
15.446	-2.7175	3.12283333333333\\
15.446	-2.7425	3.12283333333333\\
};
 
\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4472714285714	-2.54375	3.61575\\
15.4472714285714	-2.76625	3.61575\\
15.4472714285714	-2.76625	3.83825\\
15.4472714285714	-2.54375	3.83825\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.54375	3.61575\\
15.4727	-2.76625	3.61575\\
15.4727	-2.76625	3.83825\\
15.4727	-2.54375	3.83825\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.54375	3.61575\\
15.4727	-2.76625	3.61575\\
15.4472714285714	-2.76625	3.61575\\
15.4472714285714	-2.54375	3.61575\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.54375	3.83825\\
15.4727	-2.76625	3.83825\\
15.4472714285714	-2.76625	3.83825\\
15.4472714285714	-2.54375	3.83825\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.54375	3.61575\\
15.4727	-2.54375	3.83825\\
15.4472714285714	-2.54375	3.83825\\
15.4472714285714	-2.54375	3.61575\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.76625	3.61575\\
15.4727	-2.76625	3.83825\\
15.4472714285714	-2.76625	3.83825\\
15.4472714285714	-2.76625	3.61575\\
}--cycle;
\addplot3 [color=subarrayorange, only marks, mark=*, mark size = 0.1pt, mark options={solid}, line width = 0pt, mark options={solid, subarrayorange}]
 table[row sep=crcr] {%
15.446	-2.5675	3.8145\\
15.446	-2.5925	3.8145\\
15.446	-2.6175	3.8145\\
15.446	-2.6425	3.8145\\
15.446	-2.6675	3.8145\\
15.446	-2.6925	3.8145\\
15.446	-2.7175	3.8145\\
15.446	-2.7425	3.8145\\
15.446	-2.5675	3.7895\\
15.446	-2.5925	3.7895\\
15.446	-2.6175	3.7895\\
15.446	-2.6425	3.7895\\
15.446	-2.6675	3.7895\\
15.446	-2.6925	3.7895\\
15.446	-2.7175	3.7895\\
15.446	-2.7425	3.7895\\
15.446	-2.5675	3.7645\\
15.446	-2.5925	3.7645\\
15.446	-2.6175	3.7645\\
15.446	-2.6425	3.7645\\
15.446	-2.6675	3.7645\\
15.446	-2.6925	3.7645\\
15.446	-2.7175	3.7645\\
15.446	-2.7425	3.7645\\
15.446	-2.5675	3.7395\\
15.446	-2.5925	3.7395\\
15.446	-2.6175	3.7395\\
15.446	-2.6425	3.7395\\
15.446	-2.6675	3.7395\\
15.446	-2.6925	3.7395\\
15.446	-2.7175	3.7395\\
15.446	-2.7425	3.7395\\
15.446	-2.5675	3.7145\\
15.446	-2.5925	3.7145\\
15.446	-2.6175	3.7145\\
15.446	-2.6425	3.7145\\
15.446	-2.6675	3.7145\\
15.446	-2.6925	3.7145\\
15.446	-2.7175	3.7145\\
15.446	-2.7425	3.7145\\
15.446	-2.5675	3.6895\\
15.446	-2.5925	3.6895\\
15.446	-2.6175	3.6895\\
15.446	-2.6425	3.6895\\
15.446	-2.6675	3.6895\\
15.446	-2.6925	3.6895\\
15.446	-2.7175	3.6895\\
15.446	-2.7425	3.6895\\
15.446	-2.5675	3.6645\\
15.446	-2.5925	3.6645\\
15.446	-2.6175	3.6645\\
15.446	-2.6425	3.6645\\
15.446	-2.6675	3.6645\\
15.446	-2.6925	3.6645\\
15.446	-2.7175	3.6645\\
15.446	-2.7425	3.6645\\
15.446	-2.5675	3.6395\\
15.446	-2.5925	3.6395\\
15.446	-2.6175	3.6395\\
15.446	-2.6425	3.6395\\
15.446	-2.6675	3.6395\\
15.446	-2.6925	3.6395\\
15.446	-2.7175	3.6395\\
15.446	-2.7425	3.6395\\
};
 
\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4472714285714	-2.54375	4.13241666666667\\
15.4472714285714	-2.76625	4.13241666666667\\
15.4472714285714	-2.76625	4.35491666666667\\
15.4472714285714	-2.54375	4.35491666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.54375	4.13241666666667\\
15.4727	-2.76625	4.13241666666667\\
15.4727	-2.76625	4.35491666666667\\
15.4727	-2.54375	4.35491666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.54375	4.13241666666667\\
15.4727	-2.76625	4.13241666666667\\
15.4472714285714	-2.76625	4.13241666666667\\
15.4472714285714	-2.54375	4.13241666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.54375	4.35491666666667\\
15.4727	-2.76625	4.35491666666667\\
15.4472714285714	-2.76625	4.35491666666667\\
15.4472714285714	-2.54375	4.35491666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.54375	4.13241666666667\\
15.4727	-2.54375	4.35491666666667\\
15.4472714285714	-2.54375	4.35491666666667\\
15.4472714285714	-2.54375	4.13241666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.76625	4.13241666666667\\
15.4727	-2.76625	4.35491666666667\\
15.4472714285714	-2.76625	4.35491666666667\\
15.4472714285714	-2.76625	4.13241666666667\\
}--cycle;
\addplot3 [color=subarrayorange, only marks, mark=*, mark size = 0.1pt, mark options={solid}, line width = 0pt, mark options={solid, subarrayorange}]
 table[row sep=crcr] {%
15.446	-2.5675	4.33116666666667\\
15.446	-2.5925	4.33116666666667\\
15.446	-2.6175	4.33116666666667\\
15.446	-2.6425	4.33116666666667\\
15.446	-2.6675	4.33116666666667\\
15.446	-2.6925	4.33116666666667\\
15.446	-2.7175	4.33116666666667\\
15.446	-2.7425	4.33116666666667\\
15.446	-2.5675	4.30616666666667\\
15.446	-2.5925	4.30616666666667\\
15.446	-2.6175	4.30616666666667\\
15.446	-2.6425	4.30616666666667\\
15.446	-2.6675	4.30616666666667\\
15.446	-2.6925	4.30616666666667\\
15.446	-2.7175	4.30616666666667\\
15.446	-2.7425	4.30616666666667\\
15.446	-2.5675	4.28116666666667\\
15.446	-2.5925	4.28116666666667\\
15.446	-2.6175	4.28116666666667\\
15.446	-2.6425	4.28116666666667\\
15.446	-2.6675	4.28116666666667\\
15.446	-2.6925	4.28116666666667\\
15.446	-2.7175	4.28116666666667\\
15.446	-2.7425	4.28116666666667\\
15.446	-2.5675	4.25616666666667\\
15.446	-2.5925	4.25616666666667\\
15.446	-2.6175	4.25616666666667\\
15.446	-2.6425	4.25616666666667\\
15.446	-2.6675	4.25616666666667\\
15.446	-2.6925	4.25616666666667\\
15.446	-2.7175	4.25616666666667\\
15.446	-2.7425	4.25616666666667\\
15.446	-2.5675	4.23116666666667\\
15.446	-2.5925	4.23116666666667\\
15.446	-2.6175	4.23116666666667\\
15.446	-2.6425	4.23116666666667\\
15.446	-2.6675	4.23116666666667\\
15.446	-2.6925	4.23116666666667\\
15.446	-2.7175	4.23116666666667\\
15.446	-2.7425	4.23116666666667\\
15.446	-2.5675	4.20616666666667\\
15.446	-2.5925	4.20616666666667\\
15.446	-2.6175	4.20616666666667\\
15.446	-2.6425	4.20616666666667\\
15.446	-2.6675	4.20616666666667\\
15.446	-2.6925	4.20616666666667\\
15.446	-2.7175	4.20616666666667\\
15.446	-2.7425	4.20616666666667\\
15.446	-2.5675	4.18116666666667\\
15.446	-2.5925	4.18116666666667\\
15.446	-2.6175	4.18116666666667\\
15.446	-2.6425	4.18116666666667\\
15.446	-2.6675	4.18116666666667\\
15.446	-2.6925	4.18116666666667\\
15.446	-2.7175	4.18116666666667\\
15.446	-2.7425	4.18116666666667\\
15.446	-2.5675	4.15616666666667\\
15.446	-2.5925	4.15616666666667\\
15.446	-2.6175	4.15616666666667\\
15.446	-2.6425	4.15616666666667\\
15.446	-2.6675	4.15616666666667\\
15.446	-2.6925	4.15616666666667\\
15.446	-2.7175	4.15616666666667\\
15.446	-2.7425	4.15616666666667\\
};
 
\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4472714285714	-2.99575	3.09908333333333\\
15.4472714285714	-3.21825	3.09908333333333\\
15.4472714285714	-3.21825	3.32158333333333\\
15.4472714285714	-2.99575	3.32158333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.99575	3.09908333333333\\
15.4727	-3.21825	3.09908333333333\\
15.4727	-3.21825	3.32158333333333\\
15.4727	-2.99575	3.32158333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.99575	3.09908333333333\\
15.4727	-3.21825	3.09908333333333\\
15.4472714285714	-3.21825	3.09908333333333\\
15.4472714285714	-2.99575	3.09908333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.99575	3.32158333333333\\
15.4727	-3.21825	3.32158333333333\\
15.4472714285714	-3.21825	3.32158333333333\\
15.4472714285714	-2.99575	3.32158333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.99575	3.09908333333333\\
15.4727	-2.99575	3.32158333333333\\
15.4472714285714	-2.99575	3.32158333333333\\
15.4472714285714	-2.99575	3.09908333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-3.21825	3.09908333333333\\
15.4727	-3.21825	3.32158333333333\\
15.4472714285714	-3.21825	3.32158333333333\\
15.4472714285714	-3.21825	3.09908333333333\\
}--cycle;
\addplot3 [color=subarrayorange, only marks, mark=*, mark size = 0.1pt, mark options={solid}, line width = 0pt, mark options={solid, subarrayorange}]
 table[row sep=crcr] {%
15.446	-3.0195	3.29783333333333\\
15.446	-3.0445	3.29783333333333\\
15.446	-3.0695	3.29783333333333\\
15.446	-3.0945	3.29783333333333\\
15.446	-3.1195	3.29783333333333\\
15.446	-3.1445	3.29783333333333\\
15.446	-3.1695	3.29783333333333\\
15.446	-3.1945	3.29783333333333\\
15.446	-3.0195	3.27283333333333\\
15.446	-3.0445	3.27283333333333\\
15.446	-3.0695	3.27283333333333\\
15.446	-3.0945	3.27283333333333\\
15.446	-3.1195	3.27283333333333\\
15.446	-3.1445	3.27283333333333\\
15.446	-3.1695	3.27283333333333\\
15.446	-3.1945	3.27283333333333\\
15.446	-3.0195	3.24783333333333\\
15.446	-3.0445	3.24783333333333\\
15.446	-3.0695	3.24783333333333\\
15.446	-3.0945	3.24783333333333\\
15.446	-3.1195	3.24783333333333\\
15.446	-3.1445	3.24783333333333\\
15.446	-3.1695	3.24783333333333\\
15.446	-3.1945	3.24783333333333\\
15.446	-3.0195	3.22283333333333\\
15.446	-3.0445	3.22283333333333\\
15.446	-3.0695	3.22283333333333\\
15.446	-3.0945	3.22283333333333\\
15.446	-3.1195	3.22283333333333\\
15.446	-3.1445	3.22283333333333\\
15.446	-3.1695	3.22283333333333\\
15.446	-3.1945	3.22283333333333\\
15.446	-3.0195	3.19783333333333\\
15.446	-3.0445	3.19783333333333\\
15.446	-3.0695	3.19783333333333\\
15.446	-3.0945	3.19783333333333\\
15.446	-3.1195	3.19783333333333\\
15.446	-3.1445	3.19783333333333\\
15.446	-3.1695	3.19783333333333\\
15.446	-3.1945	3.19783333333333\\
15.446	-3.0195	3.17283333333333\\
15.446	-3.0445	3.17283333333333\\
15.446	-3.0695	3.17283333333333\\
15.446	-3.0945	3.17283333333333\\
15.446	-3.1195	3.17283333333333\\
15.446	-3.1445	3.17283333333333\\
15.446	-3.1695	3.17283333333333\\
15.446	-3.1945	3.17283333333333\\
15.446	-3.0195	3.14783333333333\\
15.446	-3.0445	3.14783333333333\\
15.446	-3.0695	3.14783333333333\\
15.446	-3.0945	3.14783333333333\\
15.446	-3.1195	3.14783333333333\\
15.446	-3.1445	3.14783333333333\\
15.446	-3.1695	3.14783333333333\\
15.446	-3.1945	3.14783333333333\\
15.446	-3.0195	3.12283333333333\\
15.446	-3.0445	3.12283333333333\\
15.446	-3.0695	3.12283333333333\\
15.446	-3.0945	3.12283333333333\\
15.446	-3.1195	3.12283333333333\\
15.446	-3.1445	3.12283333333333\\
15.446	-3.1695	3.12283333333333\\
15.446	-3.1945	3.12283333333333\\
};
 
\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4472714285714	-2.99575	3.61575\\
15.4472714285714	-3.21825	3.61575\\
15.4472714285714	-3.21825	3.83825\\
15.4472714285714	-2.99575	3.83825\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.99575	3.61575\\
15.4727	-3.21825	3.61575\\
15.4727	-3.21825	3.83825\\
15.4727	-2.99575	3.83825\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.99575	3.61575\\
15.4727	-3.21825	3.61575\\
15.4472714285714	-3.21825	3.61575\\
15.4472714285714	-2.99575	3.61575\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.99575	3.83825\\
15.4727	-3.21825	3.83825\\
15.4472714285714	-3.21825	3.83825\\
15.4472714285714	-2.99575	3.83825\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.99575	3.61575\\
15.4727	-2.99575	3.83825\\
15.4472714285714	-2.99575	3.83825\\
15.4472714285714	-2.99575	3.61575\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-3.21825	3.61575\\
15.4727	-3.21825	3.83825\\
15.4472714285714	-3.21825	3.83825\\
15.4472714285714	-3.21825	3.61575\\
}--cycle;
\addplot3 [color=subarrayorange, only marks, mark=*, mark size = 0.1pt, mark options={solid}, line width = 0pt, mark options={solid, subarrayorange}]
 table[row sep=crcr] {%
15.446	-3.0195	3.8145\\
15.446	-3.0445	3.8145\\
15.446	-3.0695	3.8145\\
15.446	-3.0945	3.8145\\
15.446	-3.1195	3.8145\\
15.446	-3.1445	3.8145\\
15.446	-3.1695	3.8145\\
15.446	-3.1945	3.8145\\
15.446	-3.0195	3.7895\\
15.446	-3.0445	3.7895\\
15.446	-3.0695	3.7895\\
15.446	-3.0945	3.7895\\
15.446	-3.1195	3.7895\\
15.446	-3.1445	3.7895\\
15.446	-3.1695	3.7895\\
15.446	-3.1945	3.7895\\
15.446	-3.0195	3.7645\\
15.446	-3.0445	3.7645\\
15.446	-3.0695	3.7645\\
15.446	-3.0945	3.7645\\
15.446	-3.1195	3.7645\\
15.446	-3.1445	3.7645\\
15.446	-3.1695	3.7645\\
15.446	-3.1945	3.7645\\
15.446	-3.0195	3.7395\\
15.446	-3.0445	3.7395\\
15.446	-3.0695	3.7395\\
15.446	-3.0945	3.7395\\
15.446	-3.1195	3.7395\\
15.446	-3.1445	3.7395\\
15.446	-3.1695	3.7395\\
15.446	-3.1945	3.7395\\
15.446	-3.0195	3.7145\\
15.446	-3.0445	3.7145\\
15.446	-3.0695	3.7145\\
15.446	-3.0945	3.7145\\
15.446	-3.1195	3.7145\\
15.446	-3.1445	3.7145\\
15.446	-3.1695	3.7145\\
15.446	-3.1945	3.7145\\
15.446	-3.0195	3.6895\\
15.446	-3.0445	3.6895\\
15.446	-3.0695	3.6895\\
15.446	-3.0945	3.6895\\
15.446	-3.1195	3.6895\\
15.446	-3.1445	3.6895\\
15.446	-3.1695	3.6895\\
15.446	-3.1945	3.6895\\
15.446	-3.0195	3.6645\\
15.446	-3.0445	3.6645\\
15.446	-3.0695	3.6645\\
15.446	-3.0945	3.6645\\
15.446	-3.1195	3.6645\\
15.446	-3.1445	3.6645\\
15.446	-3.1695	3.6645\\
15.446	-3.1945	3.6645\\
15.446	-3.0195	3.6395\\
15.446	-3.0445	3.6395\\
15.446	-3.0695	3.6395\\
15.446	-3.0945	3.6395\\
15.446	-3.1195	3.6395\\
15.446	-3.1445	3.6395\\
15.446	-3.1695	3.6395\\
15.446	-3.1945	3.6395\\
};
 
\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4472714285714	-2.99575	4.13241666666667\\
15.4472714285714	-3.21825	4.13241666666667\\
15.4472714285714	-3.21825	4.35491666666667\\
15.4472714285714	-2.99575	4.35491666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.99575	4.13241666666667\\
15.4727	-3.21825	4.13241666666667\\
15.4727	-3.21825	4.35491666666667\\
15.4727	-2.99575	4.35491666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.99575	4.13241666666667\\
15.4727	-3.21825	4.13241666666667\\
15.4472714285714	-3.21825	4.13241666666667\\
15.4472714285714	-2.99575	4.13241666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.99575	4.35491666666667\\
15.4727	-3.21825	4.35491666666667\\
15.4472714285714	-3.21825	4.35491666666667\\
15.4472714285714	-2.99575	4.35491666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-2.99575	4.13241666666667\\
15.4727	-2.99575	4.35491666666667\\
15.4472714285714	-2.99575	4.35491666666667\\
15.4472714285714	-2.99575	4.13241666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-3.21825	4.13241666666667\\
15.4727	-3.21825	4.35491666666667\\
15.4472714285714	-3.21825	4.35491666666667\\
15.4472714285714	-3.21825	4.13241666666667\\
}--cycle;
\addplot3 [color=subarrayorange, only marks, mark=*, mark size = 0.1pt, mark options={solid}, line width = 0pt, mark options={solid, subarrayorange}]
 table[row sep=crcr] {%
15.446	-3.0195	4.33116666666667\\
15.446	-3.0445	4.33116666666667\\
15.446	-3.0695	4.33116666666667\\
15.446	-3.0945	4.33116666666667\\
15.446	-3.1195	4.33116666666667\\
15.446	-3.1445	4.33116666666667\\
15.446	-3.1695	4.33116666666667\\
15.446	-3.1945	4.33116666666667\\
15.446	-3.0195	4.30616666666667\\
15.446	-3.0445	4.30616666666667\\
15.446	-3.0695	4.30616666666667\\
15.446	-3.0945	4.30616666666667\\
15.446	-3.1195	4.30616666666667\\
15.446	-3.1445	4.30616666666667\\
15.446	-3.1695	4.30616666666667\\
15.446	-3.1945	4.30616666666667\\
15.446	-3.0195	4.28116666666667\\
15.446	-3.0445	4.28116666666667\\
15.446	-3.0695	4.28116666666667\\
15.446	-3.0945	4.28116666666667\\
15.446	-3.1195	4.28116666666667\\
15.446	-3.1445	4.28116666666667\\
15.446	-3.1695	4.28116666666667\\
15.446	-3.1945	4.28116666666667\\
15.446	-3.0195	4.25616666666667\\
15.446	-3.0445	4.25616666666667\\
15.446	-3.0695	4.25616666666667\\
15.446	-3.0945	4.25616666666667\\
15.446	-3.1195	4.25616666666667\\
15.446	-3.1445	4.25616666666667\\
15.446	-3.1695	4.25616666666667\\
15.446	-3.1945	4.25616666666667\\
15.446	-3.0195	4.23116666666667\\
15.446	-3.0445	4.23116666666667\\
15.446	-3.0695	4.23116666666667\\
15.446	-3.0945	4.23116666666667\\
15.446	-3.1195	4.23116666666667\\
15.446	-3.1445	4.23116666666667\\
15.446	-3.1695	4.23116666666667\\
15.446	-3.1945	4.23116666666667\\
15.446	-3.0195	4.20616666666667\\
15.446	-3.0445	4.20616666666667\\
15.446	-3.0695	4.20616666666667\\
15.446	-3.0945	4.20616666666667\\
15.446	-3.1195	4.20616666666667\\
15.446	-3.1445	4.20616666666667\\
15.446	-3.1695	4.20616666666667\\
15.446	-3.1945	4.20616666666667\\
15.446	-3.0195	4.18116666666667\\
15.446	-3.0445	4.18116666666667\\
15.446	-3.0695	4.18116666666667\\
15.446	-3.0945	4.18116666666667\\
15.446	-3.1195	4.18116666666667\\
15.446	-3.1445	4.18116666666667\\
15.446	-3.1695	4.18116666666667\\
15.446	-3.1945	4.18116666666667\\
15.446	-3.0195	4.15616666666667\\
15.446	-3.0445	4.15616666666667\\
15.446	-3.0695	4.15616666666667\\
15.446	-3.0945	4.15616666666667\\
15.446	-3.1195	4.15616666666667\\
15.446	-3.1445	4.15616666666667\\
15.446	-3.1695	4.15616666666667\\
15.446	-3.1945	4.15616666666667\\
};
 
\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4472714285714	-3.44775	3.09908333333333\\
15.4472714285714	-3.67025	3.09908333333333\\
15.4472714285714	-3.67025	3.32158333333333\\
15.4472714285714	-3.44775	3.32158333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-3.44775	3.09908333333333\\
15.4727	-3.67025	3.09908333333333\\
15.4727	-3.67025	3.32158333333333\\
15.4727	-3.44775	3.32158333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-3.44775	3.09908333333333\\
15.4727	-3.67025	3.09908333333333\\
15.4472714285714	-3.67025	3.09908333333333\\
15.4472714285714	-3.44775	3.09908333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-3.44775	3.32158333333333\\
15.4727	-3.67025	3.32158333333333\\
15.4472714285714	-3.67025	3.32158333333333\\
15.4472714285714	-3.44775	3.32158333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-3.44775	3.09908333333333\\
15.4727	-3.44775	3.32158333333333\\
15.4472714285714	-3.44775	3.32158333333333\\
15.4472714285714	-3.44775	3.09908333333333\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-3.67025	3.09908333333333\\
15.4727	-3.67025	3.32158333333333\\
15.4472714285714	-3.67025	3.32158333333333\\
15.4472714285714	-3.67025	3.09908333333333\\
}--cycle;
\addplot3 [color=subarrayorange, only marks, mark=*, mark size = 0.1pt, mark options={solid}, line width = 0pt, mark options={solid, subarrayorange}]
 table[row sep=crcr] {%
15.446	-3.4715	3.29783333333333\\
15.446	-3.4965	3.29783333333333\\
15.446	-3.5215	3.29783333333333\\
15.446	-3.5465	3.29783333333333\\
15.446	-3.5715	3.29783333333333\\
15.446	-3.5965	3.29783333333333\\
15.446	-3.6215	3.29783333333333\\
15.446	-3.6465	3.29783333333333\\
15.446	-3.4715	3.27283333333333\\
15.446	-3.4965	3.27283333333333\\
15.446	-3.5215	3.27283333333333\\
15.446	-3.5465	3.27283333333333\\
15.446	-3.5715	3.27283333333333\\
15.446	-3.5965	3.27283333333333\\
15.446	-3.6215	3.27283333333333\\
15.446	-3.6465	3.27283333333333\\
15.446	-3.4715	3.24783333333333\\
15.446	-3.4965	3.24783333333333\\
15.446	-3.5215	3.24783333333333\\
15.446	-3.5465	3.24783333333333\\
15.446	-3.5715	3.24783333333333\\
15.446	-3.5965	3.24783333333333\\
15.446	-3.6215	3.24783333333333\\
15.446	-3.6465	3.24783333333333\\
15.446	-3.4715	3.22283333333333\\
15.446	-3.4965	3.22283333333333\\
15.446	-3.5215	3.22283333333333\\
15.446	-3.5465	3.22283333333333\\
15.446	-3.5715	3.22283333333333\\
15.446	-3.5965	3.22283333333333\\
15.446	-3.6215	3.22283333333333\\
15.446	-3.6465	3.22283333333333\\
15.446	-3.4715	3.19783333333333\\
15.446	-3.4965	3.19783333333333\\
15.446	-3.5215	3.19783333333333\\
15.446	-3.5465	3.19783333333333\\
15.446	-3.5715	3.19783333333333\\
15.446	-3.5965	3.19783333333333\\
15.446	-3.6215	3.19783333333333\\
15.446	-3.6465	3.19783333333333\\
15.446	-3.4715	3.17283333333333\\
15.446	-3.4965	3.17283333333333\\
15.446	-3.5215	3.17283333333333\\
15.446	-3.5465	3.17283333333333\\
15.446	-3.5715	3.17283333333333\\
15.446	-3.5965	3.17283333333333\\
15.446	-3.6215	3.17283333333333\\
15.446	-3.6465	3.17283333333333\\
15.446	-3.4715	3.14783333333333\\
15.446	-3.4965	3.14783333333333\\
15.446	-3.5215	3.14783333333333\\
15.446	-3.5465	3.14783333333333\\
15.446	-3.5715	3.14783333333333\\
15.446	-3.5965	3.14783333333333\\
15.446	-3.6215	3.14783333333333\\
15.446	-3.6465	3.14783333333333\\
15.446	-3.4715	3.12283333333333\\
15.446	-3.4965	3.12283333333333\\
15.446	-3.5215	3.12283333333333\\
15.446	-3.5465	3.12283333333333\\
15.446	-3.5715	3.12283333333333\\
15.446	-3.5965	3.12283333333333\\
15.446	-3.6215	3.12283333333333\\
15.446	-3.6465	3.12283333333333\\
};
 
\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4472714285714	-3.44775	3.61575\\
15.4472714285714	-3.67025	3.61575\\
15.4472714285714	-3.67025	3.83825\\
15.4472714285714	-3.44775	3.83825\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-3.44775	3.61575\\
15.4727	-3.67025	3.61575\\
15.4727	-3.67025	3.83825\\
15.4727	-3.44775	3.83825\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-3.44775	3.61575\\
15.4727	-3.67025	3.61575\\
15.4472714285714	-3.67025	3.61575\\
15.4472714285714	-3.44775	3.61575\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-3.44775	3.83825\\
15.4727	-3.67025	3.83825\\
15.4472714285714	-3.67025	3.83825\\
15.4472714285714	-3.44775	3.83825\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-3.44775	3.61575\\
15.4727	-3.44775	3.83825\\
15.4472714285714	-3.44775	3.83825\\
15.4472714285714	-3.44775	3.61575\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-3.67025	3.61575\\
15.4727	-3.67025	3.83825\\
15.4472714285714	-3.67025	3.83825\\
15.4472714285714	-3.67025	3.61575\\
}--cycle;
\addplot3 [color=subarrayorange, only marks, mark=*, mark size = 0.1pt, mark options={solid}, line width = 0pt, mark options={solid, subarrayorange}]
 table[row sep=crcr] {%
15.446	-3.4715	3.8145\\
15.446	-3.4965	3.8145\\
15.446	-3.5215	3.8145\\
15.446	-3.5465	3.8145\\
15.446	-3.5715	3.8145\\
15.446	-3.5965	3.8145\\
15.446	-3.6215	3.8145\\
15.446	-3.6465	3.8145\\
15.446	-3.4715	3.7895\\
15.446	-3.4965	3.7895\\
15.446	-3.5215	3.7895\\
15.446	-3.5465	3.7895\\
15.446	-3.5715	3.7895\\
15.446	-3.5965	3.7895\\
15.446	-3.6215	3.7895\\
15.446	-3.6465	3.7895\\
15.446	-3.4715	3.7645\\
15.446	-3.4965	3.7645\\
15.446	-3.5215	3.7645\\
15.446	-3.5465	3.7645\\
15.446	-3.5715	3.7645\\
15.446	-3.5965	3.7645\\
15.446	-3.6215	3.7645\\
15.446	-3.6465	3.7645\\
15.446	-3.4715	3.7395\\
15.446	-3.4965	3.7395\\
15.446	-3.5215	3.7395\\
15.446	-3.5465	3.7395\\
15.446	-3.5715	3.7395\\
15.446	-3.5965	3.7395\\
15.446	-3.6215	3.7395\\
15.446	-3.6465	3.7395\\
15.446	-3.4715	3.7145\\
15.446	-3.4965	3.7145\\
15.446	-3.5215	3.7145\\
15.446	-3.5465	3.7145\\
15.446	-3.5715	3.7145\\
15.446	-3.5965	3.7145\\
15.446	-3.6215	3.7145\\
15.446	-3.6465	3.7145\\
15.446	-3.4715	3.6895\\
15.446	-3.4965	3.6895\\
15.446	-3.5215	3.6895\\
15.446	-3.5465	3.6895\\
15.446	-3.5715	3.6895\\
15.446	-3.5965	3.6895\\
15.446	-3.6215	3.6895\\
15.446	-3.6465	3.6895\\
15.446	-3.4715	3.6645\\
15.446	-3.4965	3.6645\\
15.446	-3.5215	3.6645\\
15.446	-3.5465	3.6645\\
15.446	-3.5715	3.6645\\
15.446	-3.5965	3.6645\\
15.446	-3.6215	3.6645\\
15.446	-3.6465	3.6645\\
15.446	-3.4715	3.6395\\
15.446	-3.4965	3.6395\\
15.446	-3.5215	3.6395\\
15.446	-3.5465	3.6395\\
15.446	-3.5715	3.6395\\
15.446	-3.5965	3.6395\\
15.446	-3.6215	3.6395\\
15.446	-3.6465	3.6395\\
};
 
\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4472714285714	-3.44775	4.13241666666667\\
15.4472714285714	-3.67025	4.13241666666667\\
15.4472714285714	-3.67025	4.35491666666667\\
15.4472714285714	-3.44775	4.35491666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-3.44775	4.13241666666667\\
15.4727	-3.67025	4.13241666666667\\
15.4727	-3.67025	4.35491666666667\\
15.4727	-3.44775	4.35491666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-3.44775	4.13241666666667\\
15.4727	-3.67025	4.13241666666667\\
15.4472714285714	-3.67025	4.13241666666667\\
15.4472714285714	-3.44775	4.13241666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-3.44775	4.35491666666667\\
15.4727	-3.67025	4.35491666666667\\
15.4472714285714	-3.67025	4.35491666666667\\
15.4472714285714	-3.44775	4.35491666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-3.44775	4.13241666666667\\
15.4727	-3.44775	4.35491666666667\\
15.4472714285714	-3.44775	4.35491666666667\\
15.4472714285714	-3.44775	4.13241666666667\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=subarrayblue, fill=subarraylightblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y	z\\
15.4727	-3.67025	4.13241666666667\\
15.4727	-3.67025	4.35491666666667\\
15.4472714285714	-3.67025	4.35491666666667\\
15.4472714285714	-3.67025	4.13241666666667\\
}--cycle;
\addplot3 [color=subarrayorange, only marks, mark=*, mark size = 0.1pt, mark options={solid}, line width = 0pt, mark options={solid, subarrayorange}]
 table[row sep=crcr] {%
15.446	-3.4715	4.33116666666667\\
15.446	-3.4965	4.33116666666667\\
15.446	-3.5215	4.33116666666667\\
15.446	-3.5465	4.33116666666667\\
15.446	-3.5715	4.33116666666667\\
15.446	-3.5965	4.33116666666667\\
15.446	-3.6215	4.33116666666667\\
15.446	-3.6465	4.33116666666667\\
15.446	-3.4715	4.30616666666667\\
15.446	-3.4965	4.30616666666667\\
15.446	-3.5215	4.30616666666667\\
15.446	-3.5465	4.30616666666667\\
15.446	-3.5715	4.30616666666667\\
15.446	-3.5965	4.30616666666667\\
15.446	-3.6215	4.30616666666667\\
15.446	-3.6465	4.30616666666667\\
15.446	-3.4715	4.28116666666667\\
15.446	-3.4965	4.28116666666667\\
15.446	-3.5215	4.28116666666667\\
15.446	-3.5465	4.28116666666667\\
15.446	-3.5715	4.28116666666667\\
15.446	-3.5965	4.28116666666667\\
15.446	-3.6215	4.28116666666667\\
15.446	-3.6465	4.28116666666667\\
15.446	-3.4715	4.25616666666667\\
15.446	-3.4965	4.25616666666667\\
15.446	-3.5215	4.25616666666667\\
15.446	-3.5465	4.25616666666667\\
15.446	-3.5715	4.25616666666667\\
15.446	-3.5965	4.25616666666667\\
15.446	-3.6215	4.25616666666667\\
15.446	-3.6465	4.25616666666667\\
15.446	-3.4715	4.23116666666667\\
15.446	-3.4965	4.23116666666667\\
15.446	-3.5215	4.23116666666667\\
15.446	-3.5465	4.23116666666667\\
15.446	-3.5715	4.23116666666667\\
15.446	-3.5965	4.23116666666667\\
15.446	-3.6215	4.23116666666667\\
15.446	-3.6465	4.23116666666667\\
15.446	-3.4715	4.20616666666667\\
15.446	-3.4965	4.20616666666667\\
15.446	-3.5215	4.20616666666667\\
15.446	-3.5465	4.20616666666667\\
15.446	-3.5715	4.20616666666667\\
15.446	-3.5965	4.20616666666667\\
15.446	-3.6215	4.20616666666667\\
15.446	-3.6465	4.20616666666667\\
15.446	-3.4715	4.18116666666667\\
15.446	-3.4965	4.18116666666667\\
15.446	-3.5215	4.18116666666667\\
15.446	-3.5465	4.18116666666667\\
15.446	-3.5715	4.18116666666667\\
15.446	-3.5965	4.18116666666667\\
15.446	-3.6215	4.18116666666667\\
15.446	-3.6465	4.18116666666667\\
15.446	-3.4715	4.15616666666667\\
15.446	-3.4965	4.15616666666667\\
15.446	-3.5215	4.15616666666667\\
15.446	-3.5465	4.15616666666667\\
15.446	-3.5715	4.15616666666667\\
15.446	-3.5965	4.15616666666667\\
15.446	-3.6215	4.15616666666667\\
15.446	-3.6465	4.15616666666667\\
};

